On the Soft-Subnetwork for Few-shot Class Incremental Learning

Inspired by Regularized Lottery Ticket Hypothesis (RLTH), which hypothesizes that there exist smooth (non-binary) subnetworks within a dense network that achieve the competitive performance of the dense network, we propose a few-shot class incremental learning (FSCIL) method referred to as \emph{Soft-SubNetworks (SoftNet)}. Our objective is to learn a sequence of sessions incrementally, where each session only includes a few training instances per class while preserving the knowledge of the previously learned ones. SoftNet jointly learns the model weights and adaptive non-binary soft masks at a base training session in which each mask consists of the major and minor subnetwork; the former aims to minimize catastrophic forgetting during training, and the latter aims to avoid overfitting to a few samples in each new training session. We provide comprehensive empirical validations demonstrating that our SoftNet effectively tackles the few-shot incremental learning problem by surpassing the performance of state-of-the-art baselines over benchmark datasets.

==> 8_checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> materials/6_exper/3_concept_tsnes.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    \setlength{\tabcolsep}{-0pt}{%
    \begin{tabular}{ccc}
    \includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.1cm},clip]{images/tsne/sess0_task_id1} \\
    \includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.1cm},clip]{images/tsne/sess0_task_id2} \\
    \includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.1cm},clip]{images/tsne/sess0_task_id3} \\
    \includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.1cm},clip]{images/tsne/sess0_task_id4} \\
    %\includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.06cm},clip]{images/1_concept_biased_transfer.pdf} &
    %\includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.06cm},clip]{images/1_concept_slective_re_used.pdf} &
    %\includegraphics[height=3.0cm, trim={0.1cm 0.02cm 0.1cm 0.06cm},clip]{images/1_concept_wsns.pdf} \\ 
    
    %\makecell{\small (a) Fixed Backbone \\ \small Network} &
    %\makecell{\small (b) Biased \small Transfer} &
    %\makecell{\small (c) Selective Reuse Expansion \\ \small beyond Full Network} &
    %\makecell{\small (d) Selective Reuse Expansion \\ \small within Network (Our WSN)} \\
    \end{tabular}
    }
    \caption{\small \textbf{Subnetworks with few weights, $0.002$}}
    \label{fig:concept_comparison}
    \vspace{-0.1in}
\end{figure*}

==> materials/6_exper/5_main_cifar100_hardnet.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy on CIFAR-100 for 5-way 5-shot FSCIL with varying capasity $c$ and $c_l=1.002$.}

\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\makecell{\textbf{The gap} \\ \textbf{with cRT}}}} \\ 
\cline{2-10}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &  \\
\midrule
cRT & 65.18 & 63.89 & 60.20 & 57.23 & 53.71 & 50.39 & 48.77 & 47.29 & 45.28 & - \\
\midrule
% ---- varying capasity from 0.5 to 0.99 --------
HardNet, $c=0.80$ ,$c_l=0.002$   
& 72.22	& 67.99 & 64.32 & 60.58 & 57.45 & 54.74 & 52.92 & 50.89 & 48.65 & +3.37
\\
HardNet, $c=0.90$ ,$c_l=0.002$
& 72.78 & 68.56 & 64.93 & 61.33 & 58.2 & 55.56 & 53.59 & 51.47 & 49.26 & +3.98
\\
HardNet, $c=0.93$ ,$c_l=0.002$  
& 72.57 & 68.31 & 64.77 & 61.09 & 57.91 & 55.32 & 53.50 & 51.38 & 49.18 & +3.9
\\
HardNet, $c=\bm{0.95}$ ,$c_l=0.002$  
& \textbf{72.85} & \textbf{68.67} & \textbf{65.08} & \textbf{61.33} & \textbf{58.20} & \textbf{55.51} & \textbf{53.52} & \textbf{51.61} & \textbf{49.33} & +\textbf{4.05}
\\
HardNet, $c=0.97$ ,$c_l=0.002$  
& 72.60 & 68.51 & 64.79 & 60.99 & 57.9 & 55.08 & 53.33 & 51.31 & 49.21 & +3.93
\\
HardNet, $c=0.99$ ,$c_l=0.002$  
& 72.75 & 68.05 & 64.39 & 60.71 & 57.52 & 54.90 & 53.09 & 51.04 & 48.92 & +3.64
\\
\midrule
% ---- varying new capasity from c_l = 0.002 to 0.5 --------
HardNet, $c=0.95$, $c_l=0.002$  
& 72.85 & 68.67 & 65.08 & 61.33 & 58.20 & 55.51 & 53.52 & 51.61 & 49.33 & +4.05
\\
HardNet, $c=0.95$, $c_l=0.1$  
& \textbf{72.85} & \textbf{68.78} & \textbf{65.19}	& \textbf{61.44} & \textbf{58.29}	& \textbf{55.60}	& \textbf{53.61} & \textbf{51.70} & \textbf{49.40} & +\textbf{4.12}
\\
HardNet, $c=0.95$, $c_l=0.3$ 
& 72.85 & 68.51 & 64.98 & 61.24 & 58.13 & 55.42 & 53.44 & 51.54 & 49.26 &+3.98
\\
HardNet, $c=0.95$, $c_l=0.5$  
& 72.85	& 68.52 & 65.00	& 61.25 & 58.13 & 55.41 & 53.41 & 51.51 & 49.23 & +3.95
\\
HardNet, $c=0.95$, $c_l=0.7$  
& 72.85 & 68.63 & 65.10 & 61.33 & 58.19 & 55.50	& 53.49 & 51.59 & 49.31	& +4.03
\\
HardNet, $c=0.95$, $c_l=0.9$  
& 72.85 & 68.62 & 65.07 & 61.30 & 58.17 & 55.46 & 53.43 & 51.51 & 49.23 & +3.95
\\
\bottomrule
\end{tabular}}
\label{tab:cifar100_5way_5shot_hardnet}
\end{center}
\end{table*}

==> materials/6_exper/5_main_cifar100_temp.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy on CIFAR-100 for 5-way 5-shot FSCIL with varying temperatures $\tau$, fixed sparsity $c=0.9$ and $s=0.9$.}

\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\makecell{\textbf{The gap} \\ \textbf{with cRT}}}} \\ 
\cline{2-10}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &  \\
\midrule
cRT & 65.18 & 63.89 & 60.20 & 57.23 & 53.71 & 50.39 & 48.77 & 47.29 & 45.28 & - \\
\midrule
% ---- varying tau from 0.07 to 1.0 --------
SoftNet-c0.9-s0.9-$c_l0.102$, $\tau=0.07$  & 72.63 & 68.41 & 64.81 & 61.22 & 58.07 & 55.46 & 53.49 & 51.36 & 49.17 & +3.89 \\

SoftNet-c0.9-s0.9-$c_l0.102$, $\tau=0.1$   & 72.77 & 68.53 & 64.90 & 61.30 & 58.14 & 55.50 & 53.54 & 51.41 & 49.24 & +3.96 \\

SoftNet-c0.9-s0.9-$c_l0.102$, $\tau=\textbf{0.3}$   & \textbf{72.78} & \textbf{68.55} & \textbf{64.92} & \textbf{61.33} & \textbf{58.20} & \textbf{55.56} & \textbf{53.59} & \textbf{51.46} & \textbf{49.26} & +\textbf{3.98} \\

SoftNet-c0.9-s0.9-$c_l0.102$, $\tau=1.0$   & 72.52 & 68.33 & 64.77 & 61.17 & 58.05 & 55.39 & 53.48 & 51.39 & 49.14 & +3.85 \\
\midrule
% ---- varying tau from 0.07 to 1.0 --------
SoftNet-c0.9-s0.9-$c_l0.102$, $\tau=\textbf{0.3}$   & \textbf{72.78} & \textbf{68.55} & \textbf{64.92} & \textbf{61.33} & \textbf{58.20} & \textbf{55.56} & \textbf{53.59} & \textbf{51.46} & \textbf{49.26} & +\textbf{3.98} \\

SoftNet-c0.9-s0.9-$c_l0.5$, $~~~~\tau=0.3$   & 72.77 & 68.54 & 64.89 & 61.27 & 58.09 & 55.44 & 53.49 & 51.38 & 49.15 & +3.87 \\

SoftNet-c0.9-s0.9-$c_l0.7$, $~~~~\tau=0.3$   & 72.78 & 68.53 & 64.88 & 61.21 & 58.07 & 55.32 & 53.35 & 51.23 & 49.01 & +3.75 \\

SoftNet-c0.9-s0.9-$c_l0.9$, $~~~~\tau=0.3$   & 72.78 & 68.51 & 64.83 & 61.15 & 57.92 & 55.21 & 53.17 & 51.03 & 48.79 & +3.51 \\

\bottomrule
\end{tabular}}
\label{tab:cifar100_5way_5shot_temp}
\end{center}
\end{table*}

==> materials/6_exper/5_main_cub_10way_5shot_hardnet_baseline.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy of ResNet18 on CUB-200-2011 for 10-way 5-shot incremental learning. \underbar{Underbar} denotes the comparable results with Baseline reported by \cite{shi2021overcoming}.}

\resizebox{0.96\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{11}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\makecell{\textbf{The gap} \\ \textbf{with cRT}}}} \\ 
\cline{2-12}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11   \\
\midrule
cRT [25] \cite{shi2021overcoming} & 80.83 & 78.51 & 76.12 & 73.93 & 71.46 & 68.96 & 67.73 & 66.75 & 64.22 & 62.53 & 61.08 & - \\
Joint-training \cite{shi2021overcoming} & 80.83 & 77.57 & 74.11 & 70.75 & 68.52 & 65.97 & 64.58 & 62.22 & 60.18 & 58.49 & 56.78 & -4.30 \\
Baseline \cite{shi2021overcoming} & 80.87 & 77.15 & 74.46 & 72.26 & 69.47 & 67.18 & 65.62 & 63.68 & 61.30 & 59.72 & 58.12 & -2.96 \\
\midrule
%iCaRL [40]∗ & 79.58 & 67.63 & 64.17 & 61.80 & 58.10 & 55.51 & 53.34 & 50.89 & 48.62 & 47.34 & 45.60 & -15.48 \\
%Rebalance [20]∗ & 80.94 & 70.32 & 62.96 & 57.19 & 51.06 & 46.70 & 44.03 & 40.15 & 36.75 & 34.88 & 32.09 & -28.99 \\
%FSLL [34]∗ & 80.83 & 77.38 & 72.37 & 71.84 & 67.51 & 65.30 & 63.75 & 61.16 & 59.05 & 58.03 & 55.82 & -5.26 \\
%iCaRL [40] & 68.68 & 52.65 & 48.61 & 44.16 & 36.62 & 29.52 & 27.83 & 26.26 & 24.01 & 23.89 & 21.16 & -39.92 \\
%Rebalance [20] & 68.68 & 57.12 & 44.21 & 28.78 & 26.71 & 25.66 & 24.62 & 21.52 & 20.12 &  20.06 & 19.87 & -41.21 \\
%TOPIC [47] & 68.68 & 62.49 & 54.81 & 49.99 & 45.25 & 41.40 & 38.35 & 35.36 & 32.22 & 28.31 & 26.28 & -34.80 \\
%FSLL [34] & 72.77 & 69.33 & 65.51 & 62.66 & 61.10 & 58.65 & 57.78 & 57.26 & 55.59 & 55.39 & 54.21 & -6.87 \\
%FSLL+SS [34] & 75.63 & 71.81 & 68.16 & 64.32 & 62.61 & 60.10 & 58.82 & 58.70 & 56.45 & 56.41 & 55.82 & -5.26 \\
%IDLVQ-C [8] & 77.37 & 74.72 & 70.28 & 67.13 & 65.34 & 63.52 & 62.10 & 61.54 & 59.04 & 58.68 & 57.81 & -3.27 \\
%F2M \cite{shi2021overcoming} & 81.07 & 78.16 & 75.57 & 72.89 & 70.86 & 68.17 & 67.01 & 65.26 & 63.36 & 61.76 & 60.26 & -0.82 \\
%\midrule
FSLL \cite{mazumder2021few} & 72.77 & 69.33 & 65.51 & 62.66 & 61.10 & 58.65 & 57.78 & 57.26 & 55.59 & 55.39 & 54.21 & -6.87 \\
%FSLL+SS \cite{mazumder2021few} & 75.63 & 71.81 & 68.16 & 64.32 & 62.61 & 60.10 & 58.82 & 58.70 & 56.45 & 56.41 & 55.82 & -5.26 \\
HardNet, $c=0.70$ & 74.09 &	71.13 &	67.22 &	63.75 &	61.85 &	59.29 &	58.36 &	57.47 &	55.47 &	54.92 &	54.17 &	-6.91 \\
HardNet, $c=0.80$ & 74.84 &	71.55 &	67.67 &	64.10 &	62.51 &	60.14 &	59.13 &	58.39 & 56.58 &	56.19 &	55.63 &	-5.45\\
HardNet, $c=0.90$ & 74.81 & 71.22 &	67.31 & 63.66 &	61.95 &	59.65 &	58.96 &	58.20 &	56.45 &	56.31 &	55.66 &	-5.42 \\
HardNet, $c=0.93$ & 75.16 & 71.29 &	67.36 &	63.85 &	62.05 &	59.64 &	58.89 &	58.04 &	56.33 &	56.05 &	55.59 &	-5.49 \\
HardNet, $c=0.95$ & 74.94 & 71.16 &	67.32 &	63.66 &	61.76 &	59.43 &	58.59 &	57.71 &	55.87 & 55.61 &	55.00 & -6.08 \\
HardNet, $c=0.97$ & 74.94 & 71.14 &	67.27 &	63.69 &	61.75 &	59.15 &	58.26 &	57.23 &	55.32 &	54.89 & 54.24 &	-6.84 \\
HardNet, $c=0.99$ & 74.78 & 71.17 &	57.08 & 63.40 &	61.39 & 58.84 & 57.82 & 56.67 &	54.80 &	54.26 & 53.49 &	-7.59 \\
\midrule
SoftNet,~~$c=0.70$ & 74.06 & 71.17 & 67.24 & 63.75 & 61.85 & 59.29 & 58.37 & 57.42 & 55.47 & 54.95 & 54.17 & -6.91 \\
SoftNet,~~$c=0.80$ & 74.79 & 71.53 & 67.65 & 64.13 & 62.49 & 60.09 & 59.08 & 58.36 & 56.54 & 56.22 & 55.58 & -5.50 \\
SoftNet,~~$c=0.90$ & 74.76 & 71.23 & 67.29 & 63.65 & 61.93 & 59.65 & 58.99 & 58.20 & 56.49 & 56.29 & 55.63 & -5.45 \\
SoftNet,~~$c=0.93$ & 75.14 & 71.26 & 67.31 & 63.80 & 62.09 & 59.66 & 58.88 & 58.01 & 56.36 & 56.08 & 55.54 & -5.54 \\
SoftNet,~~$c=0.95$ & 74.90 & 71.17 & 67.35 & 63.64 & 61.75 & 59.39 & 58.57 & 57.69 & 55.91 & 55.59 & 54.98 & -6.10 \\
SoftNet,~~$c=0.97$ & 74.93 & 71.18 & 67.27 & 63.68 & 61.75 & 59.18 & 58.21 & 57.19 & 55.31 & 54.89 & 54.23 & -6.85 \\
SoftNet,~~$c=0.99$ & 74.79 & 71.12 & 57.11 & 63.37 & 61.37 & 58.79 & 57.79 & 56.71 & 54.81 & 54.26 & 53.52 & -7.56 \\
\bottomrule
\end{tabular}}
\label{tab:cub_10way_5shot}
\end{center}
\end{table*}

==> materials/6_exper/5_main_plots_cifar_hardnet_cap.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    %\setlength{\tabcolsep}{-0pt}{%
    \begin{tabular}{ccc}
    \includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/layer3_hardnet_cap_acc_cifar100.pdf} & &
    %\includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/avg_acc_0.1.pdf} & &
    \includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/layer3_hardnet_new_cap_acc_cifar100.pdf} \\
    
    \makecell{\small{(a) from $c=0.80$ to $c= 0.99$ with fixed $c_l=0.102$}} & &
    \makecell{\small{(b) from $c_l=1.01$ to $c_l=1.50$ with fixed $c=0.95$}} \\
    %\makecell{\small{(c) $\tau = 0.3$}}\\
    \end{tabular}
    %\end{adjustbox}
    \caption{\small \textbf{SoftNet on CIFAR-100 for 5-way 5-shot FSCIL:} (a) the effect of $c$ with fixed $c_l=0.102$ and (b) the effect of $c_l$ with fixed $c=0.95$. $\bigtriangledown$ and $\square$ denote base class and novel class performances, respectively.}
    \label{fig:hardnet_cap_cifar100}
\end{figure*}

==> materials/6_exper/5_main_plots_cifar_temp.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    %\setlength{\tabcolsep}{-0pt}{%
    \begin{tabular}{ccc}
    \includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/overall_avg_acc_cifar100.pdf} & &
    %\includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/avg_acc_0.1.pdf} & &
    \includegraphics[height=4.0cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/layer3_cap_acc_cifar100.pdf} \\
    
    \makecell{\small{(a) from $\tau = 0.07$ to $\tau = 1.0$ with fixed $c_l=0.102$}} & &
    \makecell{\small{(b) from $c_l=0.102$ to $c_l=0.9$ with $\tau = 0.3$}} \\
    %\makecell{\small{(c) $\tau = 0.3$}}\\
    \end{tabular}
    %\end{adjustbox}
    \caption{\small \textbf{SoftNet on CIFAR-100 for 5-way 5-shot FSCIL:} (a) the effect of $\tau$ with fixed $c_l=0.102$ and (b) the effect of $c_l$ with fixed $\tau=0.3$. $\bigtriangledown$ and $\square$ denote base class and novel class performances, respectively.}
    \label{fig:softnet_temp_cifar100}
\end{figure*}

==> materials/6_exper/5_main_plots_soft_hard.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    %\setlength{\tabcolsep}{-0pt}{%
    \begin{tabular}{cc}
    \includegraphics[height=4.6cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/cifar100/layer3_softnet_new_cap_acc_cifar100.pdf} & 
    \includegraphics[height=4.6cm, trim={0.1cm 0.02cm 0.1cm 0.2cm},clip]{images/miniImageNet/layer3_softnet_new_cap_acc_miniImageNet.pdf} \\
    
    
    \makecell{\small{(a) CIFAR-100}} &
    \makecell{\small{(b) miniImageNet}} \\
    %\makecell{\small{(c) $\tau = 0.3$}}\\
    \end{tabular}
    %\end{adjustbox}
    \caption{\small \textbf{Classification accuracy of HardNet v.s SoftNet on CIFAR-100 and miniImageNet for 5-way 5-shot FSCIL:} the overall performance depends on capacity $c$ and the softness of subnetwork and $\bigcirc$, $\bigtriangledown$, and $\square$ denote overall, base class, and novel class performances respectively. The new session performances $\square$ of SoftNet are better than those of HardNet while least forgetting base session knowledge $\bigcirc$.}
    \label{fig:hardnet_softnet}
\end{figure*}

==> materials/6_exper/5_main_table_ssl.tex <==
\begin{table*}[ht]
\small
\vspace{-0.1in}
\begin{center}
\caption{\small Performance comparison of the proposed method and baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (ACC), average capacity (CAP), and average backward transfer (BWT) across five independent runs. %CF indicates that the method suffers from the catastrophic forgetting. 
The best results are highlighted in bold. Values with $\dagger$ and $\ast$ denote reported performances from \cite{Saha2021} and \cite{Yoon2020}. We consider PackNet~\cite{mallya2018packnet} as the baseline that does not reuse learned weights from past tasks, unlike our WSN.}

\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}}&\multicolumn{3}{c}{\textbf{Permuted MNIST}}&
\multicolumn{3}{c}{\textbf{5 Datasets}}&
\multicolumn{3}{c}{\textbf{Omniglot Rotation}} \\


\midrule
&ACC (\%)&CAP (\%)&BWT&
ACC (\%)&CAP (\%)&BWT&
ACC (\%)&CAP (\%)&BWT \\
\midrule
STL&
%% One significant unita
% {97.2}~\scriptsize($\pm$ 0.1)&{$~$ 1,000.0}&-&
% {93.4}~\scriptsize($\pm$ 0.1)&{$~$ 500.0}&-&
% ~{82.1}~\scriptsize($\pm$ 0.1){\scriptsize*}&{$~$ 10,000.0}& - \\
%% Two significant units
{97.37}~\scriptsize($\pm$ 0.01)&{$~$ 1,000.0}&-&
{93.44}~\scriptsize($\pm$ 0.12)&{$~$ 500.0}&-&
~~{82.13}~\scriptsize($\pm$ 0.08)$^\ast$ &{$~$ 10,000.0}& - \\
 \midrule
FINETUNE&
%% One significant unit 
% {78.2}~\scriptsize($\pm$ 0.8)&{$~$ 100.0}&{-0.21}~\scriptsize($\pm$ 0.01)&
% {80.1}~\scriptsize($\pm$ 0.7)&{$~$ 100.0}&{-0.17}~\scriptsize($\pm$ 0.01)&
% {44.5}~\scriptsize($\pm$ 1.7)&{$~$ 100.0}&{-0.45}~\scriptsize($\pm$ 0.02) \\
%% Two significant units
{78.22}~\scriptsize($\pm$ 0.84)&{$~$ 100.0}&{-0.21}~\scriptsize($\pm$ 0.01)&
{80.06}~\scriptsize($\pm$ 0.74)&{$~$ 100.0}&{-0.17}~\scriptsize($\pm$ 0.01)&
{44.48}~\scriptsize($\pm$ 1.68)&{$~$ 100.0}&{-0.45}~\scriptsize($\pm$ 0.02) \\

EWC~\cite{Kirkpatrick2017}&
%% One significant unit 
% {92.0}~\scriptsize($\pm$ 0.6)&~~{100.0}&{-0.03}~\scriptsize($\pm$ 0.00)&
% ~~{88.6}~\scriptsize($\pm$ 0.3)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.04}~\scriptsize($\pm$ 0.01)$^\dagger$&~{68.7}~\scriptsize($\pm$ 1.9){\scriptsize*}&~~~~{100.0}{\scriptsize*}&{-} \\
{92.01}~\scriptsize($\pm$ 0.56)&~~{100.0}&{-0.03}~\scriptsize($\pm$ 0.00)&
~~{88.64}~\scriptsize($\pm$ 0.26)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.04}~\scriptsize($\pm$ 0.01)$^\dagger$&~~{68.66}~\scriptsize($\pm$ 1.92)$^\ast$&~~~~{100.0}$^\ast$&{-} \\

HAT~\cite{Serra2018}&
%% One significant unit
% {-}&{-}&{-}&
% ~~{91.3}~\scriptsize($\pm$ 0.2)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.03}~\scriptsize($\pm$ 0.00)$^\dagger$&
% {-}&{-}&{-} \\
%% Two significant units
{-}&{-}&{-}&
~~{91.32}~\scriptsize($\pm$ 0.18)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.03}~\scriptsize($\pm$ 0.00)$^\dagger$&
{-}&{-}&{-} \\

GPM~\cite{Saha2021}&
%% One significant unit
% {95.0}~\scriptsize($\pm$ 0.1)&{$~$ 100.0}&{-0.02}~\scriptsize($\pm$ 0.01)&
% ~~{91.2}~\scriptsize($\pm$ 0.2)$^\dagger$&{$~$ 100.0}&~~{-0.01}~\scriptsize($\pm$ 0.00)$^\dagger$&
% {85.2}~\scriptsize($\pm$ 0.4)&{$~$ 100.0}&{-0.01}~\scriptsize($\pm$ 0.00) \\
%% Two significant units
{94.96}~\scriptsize($\pm$ 0.07)&{$~$ 100.0}&{-0.02}~\scriptsize($\pm$ 0.01)&
~~{91.22}~\scriptsize($\pm$ 0.20)$^\dagger$&{$~$ 100.0}&~~{-0.01}~\scriptsize($\pm$ 0.00)$^\dagger$&
{85.24}~\scriptsize($\pm$ 0.37)&{$~$ 100.0}&{-0.01}~\scriptsize($\pm$ 0.00) \\

\midrule
PackNet~\cite{mallya2018packnet}&
%% One significant unit
% {96.4}~\scriptsize($\pm$ 0.0)&{$~$ 96.4}&\textbf{0.0}&
% {92.8}~\scriptsize($\pm$ 0.1)&{$~$ 82.8}&\textbf{0.0}&
% {30.7}~\scriptsize($\pm$ 1.5)&{$~$ 399.2}&\textbf{0.0} \\
%% Two significant units
{96.37}~\scriptsize($\pm$ 0.04)&{$~$ 96.38}&\cellcolor{gg}\textbf{0.0}&
{92.81}~\scriptsize($\pm$ 0.12)&{$~$ 82.86}&\cellcolor{gg}\textbf{0.0}&
{30.70}~\scriptsize($\pm$ 1.50)&{$~$ 399.2}&\cellcolor{gg}\textbf{0.0} \\ 
\midrule
WSN, $c=0.03$&% need to add per-task sparsity
%% One significant unit
% {95.0}~\scriptsize($\pm$ 0.1)&\textbf{{$~$ 20.0}~\scriptsize($\pm$ 0.1)}&\textbf{0.0}&
% {90.6}~\scriptsize($\pm$ 0.7)&\textbf{{$~$ 12.1}~\scriptsize($\pm$ 0.1)}&\textbf{0.0}& % 8.7 + 100*(1-0.78)*5/32 = 12.1 $\pm$ 0.082
% {80.7}~\scriptsize($\pm$ 2.6)&\textbf{{$~~~$ 75.9}~\scriptsize($\pm$ 1.3)}&\textbf{0.0} \\ % 7.1 + 100*(1-0.78)*100/32 = 75.9 $\pm$ 1.24
%% Two significant unit
{94.84}~\scriptsize($\pm$ 0.11)&\textbf{{$~$ 19.87}~\scriptsize($\pm$ 0.16)}&\cellcolor{gg}\textbf{0.0}&
{90.57}~\scriptsize($\pm$ 0.65)&\textbf{{$~$ 12.11}~\scriptsize($\pm$ 0.06)}&\cellcolor{gg}\textbf{0.0}& % 8.7 + 100*(1-0.78)*5/32 = 12.1 $\pm$ 0.082
{80.68}~\scriptsize($\pm$ 2.60)&\textbf{{$~~~$ 75.87}~\scriptsize($\pm$ 1.24)}&\cellcolor{gg}\textbf{0.0} \\ % 7.1 + 100*(1-0.78)*100/32 = 75.9 $\pm$ 1.24

WSN, $c=0.05$&% need to add per-task sparsity
%% One significant unit
% {95.6}~\scriptsize($\pm$ 0.2)&{$~$ 26.3}~\scriptsize($\pm$ 0.3)&\textbf{0.0}&
% {91.6}~\scriptsize($\pm$ 0.2)&{$~$ 17.3}~\scriptsize($\pm$ 0.3)&\textbf{0.0}& % 13.8 + 100*(1-0.78)*5/32 = 17.3
% \textbf{{87.3}~\scriptsize($\pm$ 0.7)}&{$~~~$ 79.8}~\scriptsize($\pm$ 1.2)&\textbf{0.0} \\ % 11.1 + 100*(1-0.78)*100/32 = 79.8
%% Two significant units
{95.65}~\scriptsize($\pm$ 0.03)&{$~$ 26.49}~\scriptsize($\pm$ 0.16)&\cellcolor{gg}\textbf{0.0}&
{91.61}~\scriptsize($\pm$ 0.21)&{$~$ 17.26}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& % 13.8 + 100*(1-0.78)*5/32 = 17.3
\textbf{{87.28}~\scriptsize($\pm$ 0.72)}&{$~~~$ 79.85}~\scriptsize($\pm$ 1.19)&\cellcolor{gg}\textbf{0.0} \\ % 11.1 + 100*(1-0.78)*100/32 = 79.8

WSN, $c=0.1$&% need to add per-task sparsity
%% One significant unit
% {96.2}~\scriptsize($\pm$ 0.1)&{$~$ 40.7}~\scriptsize($\pm$ 0.4)&\textbf{0.0}&
% {92.7}~\scriptsize($\pm$ 0.1)&{$~$ 28.0}~\scriptsize($\pm$ 0.3)&\textbf{0.0}& % 24.6 + 100*(1-0.78)*5/32 = 28.0
% {83.1}~\scriptsize($\pm$ 1.6)&{$~~~$ 83.1}~\scriptsize($\pm$ 1.6)&\textbf{0.0} \\ % 14.3 + 100*(1-0.78)*100/32 = 83.1
%% Two significant units
{96.14}~\scriptsize($\pm$ 0.03)&{$~$ 40.41}~\scriptsize($\pm$ 0.54)&\cellcolor{gg}\textbf{0.0}&
{92.67}~\scriptsize($\pm$ 0.12)&{$~$ 28.01}~\scriptsize($\pm$ 0.28)&\cellcolor{gg}\textbf{0.0}& % 24.6 + 100*(1-0.78)*5/32 = 28.0
{83.10}~\scriptsize($\pm$ 1.56)&{$~~~$ 83.08}~\scriptsize($\pm$ 1.61)&\cellcolor{gg}\textbf{0.0} \\ % 14.3 + 100*(1-0.78)*100/32 = 83.1

WSN, $c=0.3$&% need to add per-task sparsity
%% One significant unit
% \textbf{{96.5}~\scriptsize($\pm$ 0.1)}&{$~$ 77.0}~\scriptsize($\pm$ 0.5)&{\textbf{0.0}}& % 70.2 + 100*(1-0.78)*10/32 = 73.6
% {93.2}~\scriptsize($\pm$ 0.3)&{$~$ 62.3}~\scriptsize($\pm$ 0.7)&\textbf{0.0}& % 58.9 + 100*(1-0.78)*5/32 = 62.3
% {81.9}~\scriptsize($\pm$ 1.1)&{$~$ 102.2}~\scriptsize($\pm$ 0.9)&\textbf{0.0} \\ % 33.4 + 100*(1-0.78)*100/32 = 102.2
%% Two significant units
\textbf{{96.41}~\scriptsize($\pm$ 0.07)}&{$~$ 77.73}~\scriptsize($\pm$ 0.36)&{\cellcolor{gg}\textbf{0.0}}& % 70.2 + 100*(1-0.78)*10/32 = 73.6
{93.22}~\scriptsize($\pm$ 0.32)&{$~$ 62.30}~\scriptsize($\pm$ 0.69)&\cellcolor{gg}\textbf{0.0}& % 58.9 + 100*(1-0.78)*5/32 = 62.3
{81.89}~\scriptsize($\pm$ 1.15)&{$~$ ~~102.2}~\scriptsize($\pm$ 0.89)&\cellcolor{gg}\textbf{0.0} \\ % 33.4 + 100*(1-0.78)*100/32 = 102.2

WSN, $c=0.5$&% need to add per-task sparsity
%% One significant unit
% {96.3}~\scriptsize($\pm$ 0.1)&{$~$ 97.8}~\scriptsize($\pm$ 0.3)&\textbf{0.0}& 
% \textbf{{93.4}~\scriptsize($\pm$ 0.1)}&{$~$ 86.1}~\scriptsize($\pm$ 0.6)&\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
% {79.8}~\scriptsize($\pm$ 2.2)&{$~$ 121.2}~\scriptsize($\pm$ 0.5)&\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2
%% Two significant units
{96.24}~\scriptsize($\pm$ 0.11)&{$~$ 98.10}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
\textbf{{93.41}~\scriptsize($\pm$ 0.13)}&{$~$ 86.10}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{79.80}~\scriptsize($\pm$ 2.16)&{$~$ ~~121.2}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2


\midrule
MTL&
~~{96.70~\scriptsize($\pm$ 0.02)$^\dagger$}&~~{100.0}&{-}&
~~{91.54~\scriptsize($\pm$ 0.28)$^\dagger$}&~~{100.0}&{-}&
{81.23~\scriptsize($\pm$ 0.52)}&~~{100.0}&{-} \\
\bottomrule
\end{tabular}}
%\end{adjustbox}
\label{tab:main_table_ssl}
\vspace{-0.2in}
\end{center}
\end{table*}

==> materials/6_exper/5_main_table_ssl_pmnist.tex <==
\begin{table*}[ht]
\small
\vspace{-0.1in}
\begin{center}
\caption{\small Performance comparison of the proposed method and baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (ACC), average capacity (CAP), and average backward transfer (BWT) across five independent runs. %CF indicates that the method suffers from the catastrophic forgetting. 
The best results are highlighted in bold. Values with $\dagger$ and $\ast$ denote reported performances from \cite{Saha2021} and \cite{Yoon2020}. We consider PackNet~\cite{mallya2018packnet} as the baseline that does not reuse learned weights from past tasks, unlike our WSN.}

\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}}&\multicolumn{3}{c}{\textbf{Permuted MNIST-Sup}}&
\multicolumn{3}{c}{\textbf{Permuted MNIST-FlexMatch}}&
\multicolumn{3}{c}{\textbf{Permuted MNIST-Novel}} \\


\midrule
&ACC (\%)&CAP (\%)&BWT&
ACC (\%)&CAP (\%)&BWT&
ACC (\%)&CAP (\%)&BWT \\
\midrule
%STL&
%{97.37}~\scriptsize($\pm$ 0.01)&{$~$ 1,000.0}&-&
%{93.44}~\scriptsize($\pm$ 0.12)&{$~$ 500.0}&-&
%~~{82.13}~\scriptsize($\pm$ 0.08)$^\ast$ &{$~$ 10,000.0}& - \\
% \midrule
%FINETUNE&
%{78.22}~\scriptsize($\pm$ 0.84)&{$~$ 100.0}&{-0.21}~\scriptsize($\pm$ 0.01)&
%{80.06}~\scriptsize($\pm$ 0.74)&{$~$ 100.0}&{-0.17}~\scriptsize($\pm$ 0.01)&
%{44.48}~\scriptsize($\pm$ 1.68)&{$~$ 100.0}&{-0.45}~\scriptsize($\pm$ 0.02) \\

%EWC~\cite{Kirkpatrick2017}&
%{92.01}~\scriptsize($\pm$ 0.56)&~~{100.0}&{-0.03}~\scriptsize($\pm$ 0.00)&
%~~{88.64}~\scriptsize($\pm$ 0.26)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.04}~\scriptsize($\pm$ 0.01)$^\dagger$&~~{68.66}~\scriptsize($\pm$ 1.92)$^\ast$&~~~~{100.0}$^\ast$&{-} \\

%HAT~\cite{Serra2018}&
%{-}&{-}&{-}&
%~~{91.32}~\scriptsize($\pm$ 0.18)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.03}~\scriptsize($\pm$ 0.00)$^\dagger$&
%{-}&{-}&{-} \\

%GPM~\cite{Saha2021}&
%{94.96}~\scriptsize($\pm$ 0.07)&{$~$ 100.0}&{-0.02}~\scriptsize($\pm$ 0.01)&
%~~{91.22}~\scriptsize($\pm$ 0.20)$^\dagger$&{$~$ 100.0}&~~{-0.01}~\scriptsize($\pm$ 0.00)$^\dagger$&
%{85.24}~\scriptsize($\pm$ 0.37)&{$~$ 100.0}&{-0.01}~\scriptsize($\pm$ 0.00) \\

%\midrule
%PackNet~\cite{mallya2018packnet}&
%{96.37}~\scriptsize($\pm$ 0.04)&{$~$ 96.38}&\cellcolor{gg}\textbf{0.0}&
%{92.81}~\scriptsize($\pm$ 0.12)&{$~$ 82.86}&\cellcolor{gg}\textbf{0.0}&
%{30.70}~\scriptsize($\pm$ 1.50)&{$~$ 399.2}&\cellcolor{gg}\textbf{0.0} \\ 
%\midrule
%WSN, $c=0.03$&% need to add per-task sparsity
%{94.84}~\scriptsize($\pm$ 0.11)&\textbf{{$~$ 19.87}~\scriptsize($\pm$ 0.16)}&\cellcolor{gg}\textbf{0.0}&
%{90.57}~\scriptsize($\pm$ 0.65)&\textbf{{$~$ 12.11}~\scriptsize($\pm$ 0.06)}&\cellcolor{gg}\textbf{0.0}& % 8.7 + 100*(1-0.78)*5/32 = 12.1 $\pm$ 0.082
%{80.68}~\scriptsize($\pm$ 2.60)&\textbf{{$~~~$ 75.87}~\scriptsize($\pm$ 1.24)}&\cellcolor{gg}\textbf{0.0} \\ % 7.1 + 100*(1-0.78)*100/32 = 75.9 $\pm$ 1.24

%WSN, $c=0.05$&% need to add per-task sparsity
%{95.65}~\scriptsize($\pm$ 0.03)&{$~$ 26.49}~\scriptsize($\pm$ 0.16)&\cellcolor{gg}\textbf{0.0}&
%{91.61}~\scriptsize($\pm$ 0.21)&{$~$ 17.26}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& % 13.8 + 100*(1-0.78)*5/32 = 17.3
%\textbf{{87.28}~\scriptsize($\pm$ 0.72)}&{$~~~$ 79.85}~\scriptsize($\pm$ 1.19)&\cellcolor{gg}\textbf{0.0} \\ % 11.1 + 100*(1-0.78)*100/32 = 79.8

%WSN, $c=0.1$&% need to add per-task sparsity
%{96.14}~\scriptsize($\pm$ 0.03)&{$~$ 40.41}~\scriptsize($\pm$ 0.54)&\cellcolor{gg}\textbf{0.0}&
%{92.67}~\scriptsize($\pm$ 0.12)&{$~$ 28.01}~\scriptsize($\pm$ %0.28)&\cellcolor{gg}\textbf{0.0}& % 24.6 + 100*(1-0.78)*5/32 = 28.0
%{83.10}~\scriptsize($\pm$ 1.56)&{$~~~$ 83.08}~\scriptsize($\pm$ 1.61)&\cellcolor{gg}\textbf{0.0} \\ % 14.3 + 100*(1-0.78)*100/32 = 83.1

%WSN, $c=0.3$&% need to add per-task sparsity
%\textbf{{96.41}~\scriptsize($\pm$ 0.07)}&{$~$ 77.73}~\scriptsize($\pm$ 0.36)&{\cellcolor{gg}\textbf{0.0}}& % 70.2 + 100*(1-0.78)*10/32 = 73.6
%{93.22}~\scriptsize($\pm$ 0.32)&{$~$ 62.30}~\scriptsize($\pm$ 0.69)&\cellcolor{gg}\textbf{0.0}& % 58.9 + 100*(1-0.78)*5/32 = 62.3
%{81.89}~\scriptsize($\pm$ 1.15)&{$~$ ~~102.2}~\scriptsize($\pm$ 0.89)&\cellcolor{gg}\textbf{0.0} \\ % 33.4 + 100*(1-0.78)*100/32 = 102.2

%WSN, $c=0.5$, $l=0.0K$ &% need to add per-task sparsity
%{-.-}~\scriptsize($\pm$ 0.11)&{$~$ -.-}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}&
%\textbf{{-.-}~\scriptsize($\pm$ -.-)}&{$~$ -.-}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
%{-.-}~\scriptsize($\pm$ 2.16)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2
%\midrule
WSN, $c=0.5$, $l=0.010K$ &% need to add per-task sparsity
{27.06}~\scriptsize($\pm$ 0.11)&{$~$ 80.60}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& 
{16.60}~\scriptsize($\pm$ 0.11)&{$~$ 83.67}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{-.-}~\scriptsize($\pm$ 2.16)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

WSN, $c=0.5$, $l=0.020K$ &% need to add per-task sparsity
{41.91}~\scriptsize($\pm$ 0.11)&{$~$ 89.25}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& 
{22.56}~\scriptsize($\pm$ 0.11)&{$~$ 90.04}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{-.-}~\scriptsize($\pm$ 2.16)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2


WSN, $c=0.5$, $l=0.100K$ &% need to add per-task sparsity
{74.02}~\scriptsize($\pm$ 0.11)&{$~$ 89.25}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& 
{73.45}~\scriptsize($\pm$ 0.11)&{$~$ 93.30}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{-.-}~\scriptsize($\pm$ 2.16)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

\midrule

WSN, $c=0.5$, $l=1.000K$ &% need to add per-task sparsity
{87.54}~\scriptsize($\pm$ 0.11)&{$~$ 90.49}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{88.42}~\scriptsize($\pm$ 0.11)&{$~$ 90.75}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

WSN, $c=0.5$, $l=1.500K$ &% need to add per-task sparsity
{89.31}~\scriptsize($\pm$ 0.11)&{$~$ 89.82}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{89.78}~\scriptsize($\pm$ 0.11)&{$~$ 91.29}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

WSN, $c=0.5$, $l=2.000K$ &% need to add per-task sparsity
{90.02}~\scriptsize($\pm$ 0.11)&{$~$ 91.13}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{90.86}~\scriptsize($\pm$ 0.11)&{$~$ 90.49}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

WSN, $c=0.5$, $l=3.000K$ &% need to add per-task sparsity
{91.81}~\scriptsize($\pm$ 0.11)&{$~$ 90.26}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{92.30}~\scriptsize($\pm$ 0.11)&{$~$ 89.66}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

WSN, $c=0.5$, $l=4.000K$ &% need to add per-task sparsity
{91.89}~\scriptsize($\pm$ 0.11)&{$~$ 91.14}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{92.42}~\scriptsize($\pm$ 0.11)&{$~$ 91.39}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

WSN, $c=0.5$, $l=5.000K$ &% need to add per-task sparsity
{92.61}~\scriptsize($\pm$ 0.11)&{$~$ 91.75}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{92.76}~\scriptsize($\pm$ 0.11)&{$~$ 91.20}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

\midrule
WSN, $c=0.5$, $l=5.400K$ &% need to add per-task sparsity
{96.24}~\scriptsize($\pm$ 0.11)&{$~$ 98.10}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{96.24}~\scriptsize($\pm$ 0.11)&{$~$ 98.10}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
{-.-}~\scriptsize($\pm$ -.-)&{$~$ ~~-.-}~\scriptsize($\pm$ -.-)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2


%\midrule
%MTL&
%~~{96.70~\scriptsize($\pm$ 0.02)$^\dagger$}&~~{100.0}&{-}&
%~~{91.54~\scriptsize($\pm$ 0.28)$^\dagger$}&~~{100.0}&{-}&
%{81.23~\scriptsize($\pm$ 0.52)}&~~{100.0}&{-} \\
\bottomrule
\end{tabular}}
%\end{adjustbox}
\label{tab:main_table_ssl_pmnist}
\vspace{-0.2in}
\end{center}
\end{table*}

==> materials/6_exper/7_ImageNet.tex <==
\begin{table*}[ht]
\begin{center}
\caption{Classification accuracy of Subnetwork on ImageNet Dataset.}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}&\multicolumn{9}{c}{\textbf{sessions}}& \multicolumn{1}{c}{\multirow{2}{*}{\textbf{cRT}}} \\ 
%\cline{2-10}
Method & lr & scheduler & epoch & soft epoch & sparsity $c$ & $\gamma$ & accuracy   \\
\midrule
HardNet & 0.1 & [31, 61] & 90 & - & 0.1    & 1.0 & -.-   \\ 
HardNet & 0.1 & [31, 61] & 90 & - & 0.01   & 1.0 & -.-   \\ 
HardNet & 0.1 & [31, 61] & 90 & - & 0.001  & 1.0 & -.-   \\ 
HardNet & 0.1 & [31, 61] & 90 & - & 0.0001 & 1.0 & -.-   \\ \midrule

SoftNet & 0.1 & [31, 61] & 90 & 80 & 0.1 & 0.99 & -.-   \\ 
SoftNet & 0.1 & [31, 61] & 90 & 85 & 0.1 & 0.99 & -.-   \\ 
SoftNet & 0.1 & [31, 61] & 90 & 87 & 0.1 & 0.99 & -.-   \\ 
SoftNet & 0.1 & [31, 61] & 90 & 89 & 0.1 & 0.99 & -.-   \\ 

\bottomrule
\end{tabular}}
\label{tab:cifar100_5way_5shot}
\end{center}
\end{table*}

==> materials/9_backup/3_concept_comparison.tex <==
\begin{figure*}[t]
  \small
  \centering
  \vspace{-0.6in}
  \includesvg[width=0.8\linewidth]{./images/concept_comparison.svg}\\
  \vspace{-0.5in}\caption{\small \textbf{Concept Comparison} (a) Piggyback \cite{mallya2018piggyback}, and SupSup \cite{wortsman2020supermasks} find the optimal binary mask on a fixed backbone network a given task (b) PackNet \cite{mallya2018packnet} and CLNP \cite{golkar2019continual} forces the model to reuse all features and weights from previous subnetworks which causes bias in transfer of knowledge (c) APD selectively reuse and dynamically expand the full network (d) Our proposed method selectively reuse and dynamically expand subnetworks within a full network. Green edges are re-used weights}
  \label{fig:concept_comparison}
\end{figure*}


==> materials/9_backup/4_concept_figure.tex <==
\begin{figure*}[t]
  \small
  \centering
  \includesvg[width=0.8\linewidth]{images/method.svg}\\
  \vspace{-0.5in}\caption{\textbf{An illustration of Wining Subnetworks (WSN).} \modified{+ descriptions to explain this figure. [FIGURE TO BE REPLACED]}}
  \label{fig:concept_figure}
\end{figure*}


==> materials/9_backup/4_concept_wsn.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    \setlength{\tabcolsep}{-0pt}{%
    \begin{tabular}{cccc}
    \hspace{0.25in}
    \includegraphics[height=5.9cm, trim={0.1cm 0.08cm 0.1cm 0.1cm},clip]{images/illustration_wsn_t1.pdf} &\hspace{0.25in}
    \includegraphics[height=5.9cm, trim={0.1cm 0.08cm 0.1cm 0.06cm},clip]{images/illustration_wsn_t2.pdf} &\hspace{0.25in}
    \includegraphics[height=5.9cm, trim={0.1cm 0.08cm 0.1cm 0.06cm},clip]{images/illustration_wsn_t3.pdf} &\hspace{0.25in}
    \includegraphics[height=5.9cm, trim={0.1cm 0.08cm 0.1cm 0.06cm},clip]{images/illustration_wsn_t4.pdf} \\ 
    \hspace{0.25in}
    \makecell{\small (a) selected \textcolor{orange}{weights} $\hat{\bsy\theta}_{t-1}$ \\ \small at prior task} &\hspace{0.25in}
    \makecell{\small (b) forward pass \\ \small using \textcolor{Green}{reused weights}} &\hspace{0.25in}
    \makecell{\small (c) backward pass \\ \small only on \textcolor{blue}{non-used weights}} &\hspace{0.25in}
    \makecell{\small (d) selected \textcolor{blue}{weights} $\hat{\bsy\theta}_{t}$ \\ \small including subsets of \textcolor{Green}{reused weights}} \\

    \end{tabular}
    %\end{adjustbox}
    }
    \vspace{-0.1in}
    \caption{\textbf{An illustration of Winning SubNetworks (WSN):} (a) The top-c\% \textcolor{orange}{weights} $\hat{\bsy\theta}_{t-1}$ at prior task are obtained, (b) In the forward pass of a new task, WSN \textcolor{Green}{reuses weights} selected from prior tasks, (c) In the backward pass, WSN updates only \textcolor{blue}{non-used weights}, and (d) after several iterations of (b) and (c), we acquire again the top-c\% \textcolor{blue}{weights} $\hat{\bsy\theta}_{t}$ including subsets of \textcolor{Green}{reused weights}. for the new task.}
  \label{fig:concept_figure}
  \vspace{-0.1in}
\end{figure*}

==> materials/9_backup/5_acc_bar_plots.tex <==
\begin{figure}[t]
    \vspace{-0.1in}
    \centering
    \begin{adjustbox}{width=\columnwidth}
    %\setlength{\tabcolsep}{-0pt}{%
    \includegraphics[height=6.0cm, trim={1.5cm 0.1cm 1.5cm 0.1cm},clip]{images/avg_acc_bar_csnb_cifar100_10.pdf}
    %\begin{tabular}{cc}
    %\begin{tabular}{c}\includegraphics[height=8.0cm, trim={0.1cm 0.08cm 0.1cm 0.1cm},clip]{images/exper_diagram.pdf} \end{tabular} &
    %\begin{tabular}{c}
    %\includegraphics[height=12.0cm, trim={0.1cm 0.08cm 0.1cm 0.06cm},clip]{images/avg_acc_csnb_cifar100_10_c0.7.pdf}
    %\end{tabular} \\ 
    
    %{\large (a) selected} & {\large (b) forward pass} \\
    
    %\end{tabular}
    \end{adjustbox}
    %}
    % the progressively im-
    \vspace{-0.25in}
    \caption{\textbf{Comparisons on CIFAR100-Split} with \cite{deng2021flattening}: It was difficult to determine the superiority of WSN only by comparing the performances in the early stage, however, it shows the progressively better performances of WSN than others.}
  \label{fig:bar_cifar100_10}
  \vspace{-0.1in}
\end{figure}

==> materials/9_backup/5_acc_reused_per_tasks.tex <==
\begin{figure*}[htbp]
    \centering
    %\begin{adjustbox}{width=\columnwidth}
    %\setlength{\tabcolsep}{-0pt}{%
    \begin{tabular}{cc}
    
    \includegraphics[height=5.0cm, trim={0.1cm 0.1cm 0.1cm 0.1cm},clip]{images/exper_diagram.pdf}  &
    \includegraphics[height=5.0cm, trim={0.1cm 0.1cm 0.1cm 0.1cm},clip]{images/avg_acc_csnb_cifar100_10_c0.5.pdf} \\ 
    %{\large (a) selected} & {\large (b) forward pass} \\
    \end{tabular}
    %\end{adjustbox}
    %}
    \caption{\textbf{Reused Weight Performances on CIFAR-100 Split:} (left) A diagram to explain a full network of reused weights, (right) An average accuracy of reused weights; the most significant forgetting occurs from weights without reused per task; the significance of weights reused for all tasks gets lower as the number of tasks increases; In task 5, all used weights seem to be enough to infer all CIFAR-100 Split tasks since the weights reused per task catch up with the task performance.}
    \vspace{16cm} 
  \label{fig:reused_w_accuracy}
\end{figure*}

==> materials/9_backup/5_hyperparam_sweep.tex <==
\begin{figure*}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cc}
    % \includegraphics[height=3.cm]{images/5_per_task_acc_pmnist.pdf}&
    \includegraphics[height=3.cm]{images/5_per_task_acc_cifar.pdf}&
    \includegraphics[height=3.cm]{images/5_per_task_acc_5DATA.pdf} \\
    % \multicolumn{1}{c}{(a) PMNIST-MLP} & 
    \multicolumn{1}{c}{(b) SplitCIFAR100-AlexNet} &
    \multicolumn{1}{c}{(c) 5 Dataset-ResNet18}\\
    \end{tabular}}
    \caption{\footnotesize \textbf{Per task accuracy over varying $c\%$}}
    \label{fig:main_plot}
\end{figure*}

==> materials/9_backup/5_main_confusion_cifar100_10.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    \setlength{\tabcolsep}{-10pt}{%
    \begin{tabular}{cccc}
    
    \includegraphics[height=3.6cm]{images/corr_binary_csnb_cifar100_10_seed1_capacity_0.05.pdf} &~
    \includegraphics[height=3.6cm]{images/corr_binary_csnb_cifar100_10_seed1_capacity_0.1.pdf} &~ 
    \includegraphics[height=3.6cm]{images/corr_binary_csnb_cifar100_10_seed1_capacity_0.3.pdf} &~
    \includegraphics[height=3.6cm]{images/corr_binary_csnb_cifar100_10_seed1_capacity_0.5.pdf} \\ 
    
    % plot captions
    \small (a) $c=0.05$ & \small (b) $c=0.1$ & 
    \small (c) $c=0.3$ & \small (d) $c=0.5$ \\
    \end{tabular}
    %\end{adjustbox}
    }
    \caption{\footnotesize \textbf{Average Binary Map Correlation} on Sequence of CIFAR-100 Split Experiments: the binary maps get overlapped with prior ones as the number of tasks increases..}
    \label{fig:main_cifar100_conf}
\end{figure*}

==> materials/9_backup/5_main_confusion_cifar100_100.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    \setlength{\tabcolsep}{-10pt}{%
    \begin{tabular}{cccc}
    
    \includegraphics[height=3.57cm]{images/corr_binary_csnb_cifar100_100_seed1_capacity_0.05.pdf} &~\;
    \includegraphics[height=3.57cm]{images/corr_binary_csnb_cifar100_100_seed1_capacity_0.1.pdf} &~\; 
    \includegraphics[height=3.57cm]{images/corr_binary_csnb_cifar100_100_seed1_capacity_0.3.pdf} &~\;
    \includegraphics[height=3.57cm]{images/corr_binary_csnb_cifar100_100_seed1_capacity_0.5.pdf} \\ 
    
    % plot captions
    \small (a) $c=0.05$ & \small (b) $c=0.1$ & 
    \small (c) $c=0.3$ & \small (d) $c=0.5$ \\
    \end{tabular}
    %\end{adjustbox}
    }
    \caption{\footnotesize \textbf{Average Binary Map Correlation} on Sequence of CIFAR-100 Superclass Experiments: the binary maps get overlapped with prior ones as the number of tasks increases..}
    \label{fig:main_cifar100sc_conf}
\end{figure*}

==> materials/9_backup/5_main_confusion_tinyimagenet.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    \setlength{\tabcolsep}{-9pt}{%
    \begin{tabular}{cccc}
    
    \includegraphics[height=3.53cm]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.05.pdf} &~~
    \includegraphics[height=3.53cm]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.1.pdf} &~~
    \includegraphics[height=3.53cm]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.3.pdf} &~~
    \includegraphics[height=3.53cm]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.5.pdf} \\ 
    
    % plot captions
    \small (a) $c=0.05$ & \small (b) $c=0.1$ & 
    \small (c) $c=0.3$ & \small (d) $c=0.5$ \\
    \end{tabular}
    %\end{adjustbox}
    }
    \caption{\footnotesize \textbf{Average Binary Map Correlation} on Sequence of TinyImageNet Dataset Experiments: the binary maps get overlapped with prior ones as the number of tasks increases..}
    \label{fig:main_tinyimg_conf}
\end{figure*}

==> materials/9_backup/5_main_confusion_tinyimagenet2.tex <==
\begin{figure}[t]
    \centering
    \vspace{-0.1in}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    % we prepare the figure 
    \includegraphics[height=3.2cm]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.1.pdf} & 
    \includegraphics[height=3.2cm]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.5.pdf} \\
    
    \small (a) WSN, $c=0.1$  &\small (b) WSN, $c=0.5$
    
    %\vspace{-0.05in}
    %\multicolumn{2}{c}{\small (a) Per Task Accuracy over Varying $c$} &
    %\multicolumn{3}{c}{\small (b) \% Weights used per Layer over Increasing No. of Tasks}
    \end{tabular}}
    
    \caption{\footnotesize \textbf{Task-wise Binary Map Correlations} on TinyImageNet: $c=0.5$ WSN reused task weights more than $c=0.1$ ones as shown in higher correlation results than others.}
    \label{fig:main_confs_wsn_packnet}
    \vspace{-0.12in}
\end{figure}

==> materials/9_backup/5_main_confusions.tex <==
\begin{figure}[ht]
    \centering
    % \vspace{-0.1in}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    % we prepare the figure 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_Omniglot Rotation_seed_1_capacity_2_PackNet.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_Omniglot Rotation_seed_5_capacity_5.pdf} \\
    \small (a) PackNet & \small (b) WSN, $c = 0.05$ \\
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.1.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/corr_binary_csnb_tiny_data_seed1_capacity_0.5.pdf} \\
    \small (c) WSN, $c=0.1$  & \small (d) WSN, $c=0.5$
    \end{tabular}}
    \caption{\footnotesize \textbf{Task-wise Binary Map Correlations} on Omniglot Rotation (Top row) and TinyImageNet (Bottom row). WSN reuses the weights while PackNet does not. WSN with $c=0.5$ reuses task weights more than the case of $c=0.1$ as shown in higher correlation results than others.}
    \label{fig:main_confs_wsn_packnet}
    \vspace{-0.15in}
\end{figure}


==> materials/9_backup/5_main_plots.tex <==
\begin{figure*}[ht]
    \centering
    \setlength{\tabcolsep}{-15pt}{%
-    \begin{tabular}{cccc}
    \includegraphics[height=3.5cm]{images/5_cf_cifar.pdf} &
    \includegraphics[height=3.5cm]{images/5_acc_vs_cap_pmnist.pdf} &
    \includegraphics[height=3.5cm]{images/5_acc_vs_cap_5data.pdf} &
    \includegraphics[height=3.5cm]{images/5_used_weights_vs_num_tasks.pdf} &
    % \includegraphics[height=3.5cm]{images/5_acc_vs_sparsity.pdf}
     \\
     \small (a) Catastrophic Forgetting &
    \multicolumn{2}{c}{\small (b) Accuracy over Model Size} &
    % \multicolumn{2}{c}{(b) Catastrophic Forgetting during training} \\
    \small(c) Scalability to Large No. of Tasks  
    \end{tabular}}
    \caption{\footnotesize \textbf{Performance}}
    \label{fig:main_plots}
\end{figure*}

==> materials/9_backup/5_main_plots_2.tex <==
\begin{figure*}[ht]
    \centering
    \setlength{\tabcolsep}{-25pt}{%
    \begin{tabular}{ccccc}
    \includegraphics[height=3.5cm]{images/5_per_task_acc_cifar.pdf} &
    \includegraphics[height=3.5cm]{images/5_per_task_acc_5DATA.pdf} &
    \includegraphics[height=3.5cm]{images/5_per_layer_sparsity_pmnist.pdf} &
    \includegraphics[height=3.5cm]{images/5_per_layer_sparsity_cifar.pdf} &
    \includegraphics[height=3.5cm]{images/5_per_layer_sparsity_5DATA.pdf} \\
    %\includegraphics[height=3.5cm]{images/5_acc_vs_sparsity.pdf}
    \multicolumn{2}{c}{\small (a) Per Task Accuracy over Varying $c$} &
    \multicolumn{3}{c}{\small (b) \% Weights used per Layer over Increasing No. of Tasks} 
    \end{tabular}}
    \caption{\footnotesize \textbf{Performance}}
    \label{fig:main_plots2}
\end{figure*}

==> materials/9_backup/5_main_plots_acc_vs_cap.tex <==
\begin{figure}[ht]
    \centering
    \vspace{-0.1in}
    \renewcommand{\arraystretch}{1}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    \includegraphics[width=.5\columnwidth]{images/5_acc_vs_cap_5data_new_w_dots_no_title.pdf} &
    \includegraphics[width=.5\columnwidth]{images/5_acc_vs_cap_omniglot_rotation_new_w_dots_no_title.pdf} \\
    % \vspace{-0.06in}
    \small (a) 5-Dataset - ResNet-18 & \small (b) Omniglot Rotation - LeNet\\
    % \vspace{-0.06in}
    %\multicolumn{2}{c}{\small (a) Per Task Accuracy over Varying $c$} &
    %\multicolumn{3}{c}{\small (b) \% Weights used per Layer over Increasing No. of Tasks}
    \end{tabular}}
    % \vspace{-0.15in}
    %\caption{\footnotesize \textbf{Accuracy over Total Capacity Usage}: The performances of WSN gets better than others as total model capacities increase - WSN's accuracy is higher than PackNet's approximately at 80\% total capacity usage on 5-Dataset and WSN outperformed others at 80\% total capacity usage on Omniglot Rotation.}
    \caption{\footnotesize \textbf{Accuracy over Total Capacity Usage}: The performances of WSN gets better than others as total model capacities increase, and then, saturated approximately at 80 \%.}
    
    \label{fig:acc_vs_cap}
\vspace{-0.1in}
\end{figure}

==> materials/9_backup/5_main_plots_capacity.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cccc}
    
    \includegraphics[width=0.25\textwidth]{images/avg_all_capa_csnb_tiny_data.pdf} & 
    % \hspace{0.08in}
    \includegraphics[width=0.25\textwidth]{images/avg_layer_all_capa_csnb_tiny_data_c0.1_conv.pdf} &
    % \hspace{0.08in} 
    \includegraphics[width=0.25\textwidth]{images/avg_layer_all_capa_csnb_tiny_data_c0.1_conv_linear.pdf} & 
    % \hspace{0.08in}
    \includegraphics[width=0.25\textwidth]{images/avg_layer_all_capa_csnb_tiny_data_c0.1_linear.pdf} \\ 
    
    % plot captions
    \small (a) Capacities over $c$ & \small (b) Conv1 vs. Conv4 Layer &
    \small (c) Conv4 vs. Linear2 Layer & \small (d) Linear1 vs. Linear2 Layer \\
    %\includegraphics[width=\linewidth]{images/avg_all_capa_csnb_tiny_data.pdf} &
    %\includegraphics[width=\linewidth]{images/avg_layer_all_capa_csnb_tiny_data_c0.1_conv.pdf} \\ 
    %\small (a) Capacities over $c$ & \small (b) Layer-wise-Capacities: conv1 v.s. conv4 layers \\
    %\includegraphics[width=\linewidth]{images/avg_layer_all_capa_csnb_tiny_data_c0.1_conv_linear.pdf} &
    %\includegraphics[width=\linewidth]{images/avg_layer_all_capa_csnb_tiny_data_c0.1_linear.pdf} \\ 
    %\small (c) Layer-wise-Capacities: conv4 v.s. linear2 layers & \small (d) Layer-wise-Capacities: linear1 v.s. linear2 layesr \\
    %\multicolumn{2}{c}{\small (a) } & \multicolumn{3}{c}{\small (b)}
    \end{tabular}
    %\end{adjustbox}
    }
    \caption{\footnotesize \textbf{The 4 Conv \& 3 FC Layer-wise Average Capacities} on Sequence of TinyImageNet Dataset Experiments. (a) The proportion of reused weights per task depends on $c$ value, and the proportion of reused weights for all tasks tend to be decreasing, (b) The capacity of Conv4 with high variance is greater than Conv1 with low variance and the Conv4 proportion of reused weights for all tasks are smaller than the Conv1, (c) The capacity of Conv4 with high variance is greater than Liner2 with low variance and the Conv4 proportion of reused weights for all tasks are smaller than the Linear2, and (d) The capacity of Linear1 is greater than Linear2 in the early task learning stage, and the Linear1 proportion of reused weights for all tasks are smaller than the Linear2 in the early task learning stage. From (b), (c), and (d), the proportion of reused weights per task tends to be progressively saturated to $c=0.1$ value.}
    
    %\caption{\footnotesize \textbf{The 4 Conv \& 3 FC Layer-wise Average Capacities} on Sequence of TinyImageNet Dataset Experiments. (a) Capacities of $c=0.1$: the $c$ value determines both initial task capacity and progressive task capacity; the proportion of reused weights per task depends on $c$ value, and the proportion of reused weights for all tasks tend to be decreasing, (b) Conv1 vs. Conv4: the capacity of Conv4 with high variance is greater than Conv1 with low variance and the Conv4 proportion of reused weights for all tasks are smaller than the Conv1, (c) Conv4 vs. Linear2: the capacity of Conv4 with high variance is greater than Liner2 with low variance and the Conv4 proportion of reused weights for all tasks are smaller than the Linear2, and (d) Linear1 vs. Linear2: the capacity of Linear1 is greater than Linear2 in the early task learning stage, and the Linear1 proportion of reused weights for all tasks are smaller than the Linear2 in the early task learning stage. From (b), (c), and (d), the proportion of reused weights per task tends to be progressively saturated to $c=0.1$ value.}
    \label{fig:main_tinyimg_all_capa_plots}
\end{figure*}

==> materials/9_backup/5_main_plots_capacity_acc.tex <==
\begin{figure*}[ht]
    %\vspace{-0.1in}
    \centering
    % \resizebox{\textwidth}{!}{
    \setlength{\tabcolsep}{-10pt}{%
    \begin{tabular}{cccc}

    \includegraphics[height=3.13cm,trim={0.1cm 0.1cm 0.1cm 0.1cm},clip]{images/exper_diagram.pdf} & ~~~ 
    \includegraphics[height=3.13cm,trim={0.1cm 0.1cm 0.1cm 0.1cm},clip]{images/avg_all_capa_csnb_tiny_data.pdf} & ~~~ 
    \includegraphics[height=3.13cm,trim={0.1cm 0.1cm 0.1cm 0.1cm},clip]{images/avg_acc_csnb_tiny_data_c0.1.pdf} & ~~~
    \includegraphics[height=3.13cm,trim={0.1cm 0.1cm 0.1cm 0.1cm},clip]{images/avg_acc_csnb_tiny_data_layer_c0.1.pdf} \\ 
    
    % \includegraphics[height=3.0cm, trim={0.1cm 0.08cm 0.1cm 0.1cm},clip]{images/exper_diagram.pdf} & ~\hspace{0.005in}
    % \includegraphics[height=3.34cm]{images/avg_all_capa_csnb_tiny_data.pdf} & \hspace{-0.12in} 
    % \includegraphics[height=3.34cm]{images/avg_acc_csnb_tiny_data_c0.1.pdf} & \hspace{-0.12in} 
    % \includegraphics[height=3.34cm]{images/avg_acc_csnb_tiny_data_layer_c0.1.pdf} \\ 
    
    %\begin{tabular}{c}\includegraphics[height=10.0cm, trim={0.1cm 0.08cm 0.1cm 0.1cm},clip]{images/exper_diagram.pdf} \end{tabular} &
    %\begin{tabular}{c}
    %\includegraphics[height=12.0cm, trim={0.1cm 0.08cm 0.1cm 0.06cm},clip]{images/avg_acc_csnb_tiny_data_c0.1.pdf}
    %\end{tabular} 
    %&
    %\begin{tabular}{c}
    %\includegraphics[height=12.0cm, trim={0.1cm 0.08cm 0.1cm 0.06cm},clip]{images/avg_acc_csnb_tiny_data_c0.1.pdf}
    %\end{tabular}
    %&
    %\begin{tabular}{c}
    %\includegraphics[height=12.0cm, trim={0.1cm 0.08cm 0.1cm 0.06cm},clip]{images/avg_acc_csnb_tiny_data_c0.1.pdf}
    %\end{tabular}
    %\\ 
    
    % plot captions
    \small (a) A Diagram of Capacities 
    & \small (b) Capacities over $c$ 
    & \small (c) Accuracy of Reused Weights 
    & \small (d) Accuracy w/o Reused Weights \\
    \vspace{-0.2in}
    \end{tabular}
    }
    % }
    
    
    %\caption{\footnotesize \textbf{The 4 Conv \& 3 FC Layer-wise Average Capacity-Accuracy} on Sequence of TinyImageNet Dataset Experiments. (a) A diagram to explain a full network of reused weights (b) Capacities of $c=0.1$ except to binary maps: the $c$ value determines both initial task capacity and progressive task capacity; the proportion of reused weights per task depends on $c$ value, and the proportion of reused weights for all prior tasks tend to be decreasing, (c) An average accuracy of reused weights; the most significant forgetting occurs from weights without reused per task; the significance of weights reused for all tasks gets lower as the number of tasks increases; from task 7, all used weights seem to be enough to infer all tasks since the weights reused per task catch up with the task performance, and (d) The Observations of layer-wise forgetting caused by removing reused weights per task of network layers and performance drops significantly without using weights reused per task of conv1 layer.}
    
    %\caption{\footnotesize \textbf{Layer-wise Analysis} on TinyImageNet Dataset Experiments: (a) a diagram explains a full network of reused weights (b) Capacities of $c=0.1$ except to binary maps: the $c$ value determines both initial task capacity and progressive task capacities of reused weights per task and reused weights for all prior tasks, (c) the most significant forgetting occurs from weights without reused per task; the significance of weights reused for all tasks gets lower and from task 7, all used weights seem to be enough to infer all tasks since the weights reused per task catch up with the task performance, and (d) we inspected a layer-wise forgetting caused by removing reused weights per task on the trained model and observed performance drops significantly at conv1 layer.}
    
    \caption{\footnotesize \textbf{Layer-wise Analysis} on TinyImageNet Dataset Experiments: (a) Weights reusability within a full network, (b) Capacities except to binary maps are determined by $c=0.1$, (c) The most significant forgetting occurs from weights without reused per task; the significance of weights reused for all tasks gets lower and from task 7, all used weights seem to be enough to infer all tasks, and (d) We inspected a layer-wise forgetting caused by removing reused weights per task on the trained model and observed performance drops significantly at conv1 layer.}
    
    \label{fig:main_tinyimg_all_acc_plots}
    \vspace{-0.15in}
\end{figure*}

==> materials/9_backup/5_main_plots_tinyimagenet2.tex <==
\begin{figure}[t]
    \centering
    % \begin{sc}
    % \resizebox{\colum}{!}{
    % \vspace{-0.1in}
    \setlength{\tabcolsep}{-7pt}{%
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{cc}
    
    %\includegraphics[width=0.5\columnwidth]{images/avg_acc_csnb_tiny_data.pdf} & %\hspace{-0.1in}
    %\includegraphics[width=0.5\columnwidth]{images/avg_bit_capa_csnb_tiny_data_huffman.pdf} \\
    
    \includegraphics[height=2.96cm,trim={0.3cm 0.1cm 0.1cm 0.1cm},clip]{images/avg_acc_csnb_tiny_data.pdf} &\;\; 
    \includegraphics[height=2.96cm,trim={0.1cm 0.1cm 0.1cm 0.1cm},clip]{images/avg_bit_capa_csnb_tiny_data_huffman.pdf} \\
    
    \small (a) Per Task Accuracy over $c$ & \small (b) Model Capacity
    % \vspace{-0.1in}
    \end{tabular}}
    % }
    \caption{\footnotesize \textbf{Performances and Compressed Capacities}: Sequence of TinyImageNet Dataset Experiments: (a) Setting $c=0.1$ shows generalized performances over others and (b) Within 40 tasks, the 7-bits compressed model increase its capacity the least.}
    % \end{sc}
    \label{fig:main_tinyimg_plots}
    \vspace{-0.1in}
\end{figure}

==> materials/9_backup/5_main_plots_tinyimgnet.tex <==
\begin{figure*}[ht]
    \centering
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{ccccc}
    \includegraphics[width=0.33333\textwidth]{images/avg_acc_csnb_tiny_data.pdf}  & 
    % \hspace{0.6in}
    \includegraphics[width=0.33333\textwidth]{images/avg_comp_rate_csnb_tiny_data_huffman.pdf} &
    % \hspace{0.6in}
    \includegraphics[width=0.33333\textwidth]{images/avg_bit_capa_csnb_tiny_data_huffman.pdf} \\
    
    
    \small (a) Per Task Accuracy over $c$ & \small (b) N-Bit-wise-Compression Rate & \small (c) Progressive Capacities of Models
    
    %\multicolumn{2}{c}{\small (a) Per Task Accuracy over Varying $c$} &
    %\multicolumn{3}{c}{\small (b) \% Weights used per Layer over Increasing No. of Tasks}
    \end{tabular}}
    \caption{\footnotesize \textbf{Performances and Compressed Capacities} - Sequence of TinyImageNet Dataset Experiments. (a) The $c=0.1$ shows generalized performances over others, (b) With fixed $c=0.1$, we investigate the bit-wise Huffman compression rate and observe that as the number of bits to compress increases the average compression rate gets higher, and (c) We compared the model capacity with the model capacity + the compressed binary masks over varying bits. Within the 40-tasks, the 7-bits compressed capacities are the least increasing along with the $c=0.1$ model capacity.}
    \label{fig:app_main_tinyimg_plots}
\end{figure*}

==> materials/9_backup/5_main_table.tex <==
\begin{table*}[t]
\tiny
\begin{center}
\caption{\small Performance comparison of the proposed method and other baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (Accuracy) and average forgetting (Forgetting) across $5$ independent runs. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Values with $\dagger$ $~$ denote reported performances from \cite{Saha2021}. PackNet~\cite{mallya2018packnet} is baseline.}

\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Method}}&\multicolumn{2}{c}{\textbf{Permuted MNIST}} & \multicolumn{2}{c}{\textbf{Split CIFAR-100}} & \multicolumn{2}{c}{\textbf{5 Datasets}} \\


\midrule
& CF & Accuracy & Capacity Used & Accuracy & Capacity Used & Accuracy & Capacity Used\\
\midrule
STL & $\bsy\times$ &
{\scriptsize 97.6} ($\pm$ 0.10) & {\scriptsize 1000.0} \%&
{\scriptsize 70.9} ($\pm$ 0.38) & {\scriptsize 1000.0} \%&
{\scriptsize 90.7} ($\pm$ 0.53) & {\scriptsize 500.0} \%\\
 \midrule
FINETUNE&  \checkmark &
{\scriptsize 62.5} ($\pm$ 2.96) & {\scriptsize 100.0} \%&
{\scriptsize 13.2} ($\pm$ 0.54) & {\scriptsize 100.0} \%&
{\scriptsize 36.8} ($\pm$ 2.25) & {\scriptsize 100.0} \%\\
HAT~\cite{Serra2018} &  \checkmark &
{\scriptsize -}  & {\scriptsize -} &
{\scriptsize 72.0} $\dagger$ & {\scriptsize 100.0} \%&
{\scriptsize 88.6} $\dagger$ & {\scriptsize 100.0} \%\\
% APD~\cite{Yoon2020}  & \checkmark &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%\\

AGS-CL~\cite{Jung2020} & \checkmark &
{\scriptsize 91.1} ($\pm$ 0.71) & {\scriptsize 100.0} \%&
{\scriptsize 49.6} ($\pm$ 1.89) & {\scriptsize 100.0} \%&
{\scriptsize -}  & -\\

GPM~\cite{Saha2021} & \checkmark &
% {\scriptsize 92.9} ($\pm$ 0.20) & {\scriptsize x.xx} \%&
{\scriptsize 93.9} $\dagger$ & {\scriptsize 100.0} \%&
{\scriptsize 72.5} $\dagger$ & {\scriptsize 100.0} \%&
{\scriptsize 91.3} $\dagger$ & {\scriptsize 100.0} \%\\
\cmidrule{1-8}
PackNet~\cite{mallya2018packnet}  & $\bsy\times$ &
%\textbf{{\scriptsize 95.9} ($\pm$ 0.05)} & {\scriptsize $~$ 96.8} \%& % 0.655 + 10*1/32
{\scriptsize 94.5} ($\pm$ 0.05) & {\scriptsize $~$ 72.1} \%& % 0.408 + 10*1/32
{\scriptsize 58.3} ($\pm$ 0.46) & {\scriptsize 131.2} \%& % 0.999 + 10*1/32
{\scriptsize 89.0} ($\pm$ 0.21) & {\scriptsize 115.4} \%\\ % 0.998 + 5 * 1/32
% LL-Ticket~\cite{longliveticket}  & $\bsy\times$ &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%\\
\cmidrule{1-8}
CST (Ours) $c=0.03$ & $\bsy\times$ &
{\scriptsize 92.7} ($\pm$ 0.06) & \textbf{{\scriptsize $~$ 37.4}} \%&
{\scriptsize 65.6} ($\pm$ 0.63) & \textbf{{\scriptsize $~$ 39.4}} \%&
{\scriptsize 90.1} ($\pm$ 0.10) & \textbf{{\scriptsize $~$ 24.2}} \%\\
CST (Ours) $c=0.1$ & $\bsy\times$ &
{\scriptsize 93.9} ($\pm$ 0.09) & {\scriptsize $~$ 46.3} \%&
{\scriptsize 72.2} ($\pm$ 0.36) & {\scriptsize $~$ 56.2} \%&
{\scriptsize 91.3} ($\pm$ 0.13) & {\scriptsize $~$ 39.9} \%\\
CST (Ours) $c=0.3$ & $\bsy\times$ &
{\scriptsize 94.7} ($\pm$ 0.07) & {\scriptsize $~$ 68.3} \%& \textbf{{\scriptsize 73.5} ($\pm$ 0.40)} & {\scriptsize $~$ 97.4} \%& \textbf{{\scriptsize 91.7} ($\pm$ 0.23)} & {\scriptsize $~$ 72.9} \%\\
CST (Ours) $c=0.5$ & $\bsy\times$ &
\textbf{{\scriptsize 94.8} ($\pm$ 0.02)} & {\scriptsize $~$ 88.9} \%& {\scriptsize 72.5 ($\pm$ 0.92)} & {\scriptsize 111.0} \%& {\scriptsize 91.5} ($\pm$ 0.13) & {\scriptsize $~$ 95.8} \%\\
\cmidrule{1-8}
MTL &$\bsy\times$& {\scriptsize 96.7 $\dagger$} & {\scriptsize 100.0} \%& {\scriptsize 79.6 $\dagger$} & {\scriptsize 100.0} \%& {\scriptsize 91.5 $\dagger$} & {\scriptsize 100.0} \%\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main_table}
\end{center}
\end{table*}




==> materials/9_backup/5_main_table_larger.tex <==
\begin{table*}[ht]
\small
\vspace{-0.1in}
\begin{center}
\caption{\small Performance comparison of the proposed method and baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (ACC), average capacity (CAP), and average backward transfer (BWT) across five independent runs. %CF indicates that the method suffers from the catastrophic forgetting. 
The best results are highlighted in bold. Values with $\dagger$ and $\ast$ denote reported performances from \cite{Saha2021} and \cite{Yoon2020}. We consider PackNet~\cite{mallya2018packnet} as the baseline that does not reuse learned weights from past tasks, unlike our WSN.}

\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}}&\multicolumn{3}{c}{\textbf{Permuted MNIST}}&
\multicolumn{3}{c}{\textbf{5 Datasets}}&
\multicolumn{3}{c}{\textbf{Omniglot Rotation}} \\


\midrule
&ACC (\%)&CAP (\%)&BWT&
ACC (\%)&CAP (\%)&BWT&
ACC (\%)&CAP (\%)&BWT \\
\midrule
STL&
%% One significant unit
% {97.2}~\scriptsize($\pm$ 0.1)&{$~$ 1,000.0}&-&
% {93.4}~\scriptsize($\pm$ 0.1)&{$~$ 500.0}&-&
% ~{82.1}~\scriptsize($\pm$ 0.1){\scriptsize*}&{$~$ 10,000.0}& - \\
%% Two significant units
{97.37}~\scriptsize($\pm$ 0.01)&{$~$ 1,000.0}&-&
{93.44}~\scriptsize($\pm$ 0.12)&{$~$ 500.0}&-&
~~{82.13}~\scriptsize($\pm$ 0.08)$^\ast$ &{$~$ 10,000.0}& - \\
 \midrule
FINETUNE&
%% One significant unit 
% {78.2}~\scriptsize($\pm$ 0.8)&{$~$ 100.0}&{-0.21}~\scriptsize($\pm$ 0.01)&
% {80.1}~\scriptsize($\pm$ 0.7)&{$~$ 100.0}&{-0.17}~\scriptsize($\pm$ 0.01)&
% {44.5}~\scriptsize($\pm$ 1.7)&{$~$ 100.0}&{-0.45}~\scriptsize($\pm$ 0.02) \\
%% Two significant units
{78.22}~\scriptsize($\pm$ 0.84)&{$~$ 100.0}&{-0.21}~\scriptsize($\pm$ 0.01)&
{80.06}~\scriptsize($\pm$ 0.74)&{$~$ 100.0}&{-0.17}~\scriptsize($\pm$ 0.01)&
{44.48}~\scriptsize($\pm$ 1.68)&{$~$ 100.0}&{-0.45}~\scriptsize($\pm$ 0.02) \\

EWC~\cite{Kirkpatrick2017}&
%% One significant unit 
% {92.0}~\scriptsize($\pm$ 0.6)&~~{100.0}&{-0.03}~\scriptsize($\pm$ 0.00)&
% ~~{88.6}~\scriptsize($\pm$ 0.3)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.04}~\scriptsize($\pm$ 0.01)$^\dagger$&~{68.7}~\scriptsize($\pm$ 1.9){\scriptsize*}&~~~~{100.0}{\scriptsize*}&{-} \\
{92.01}~\scriptsize($\pm$ 0.56)&~~{100.0}&{-0.03}~\scriptsize($\pm$ 0.00)&
~~{88.64}~\scriptsize($\pm$ 0.26)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.04}~\scriptsize($\pm$ 0.01)$^\dagger$&~~{68.66}~\scriptsize($\pm$ 1.92)$^\ast$&~~~~{100.0}$^\ast$&{-} \\

HAT~\cite{Serra2018}&
%% One significant unit
% {-}&{-}&{-}&
% ~~{91.3}~\scriptsize($\pm$ 0.2)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.03}~\scriptsize($\pm$ 0.00)$^\dagger$&
% {-}&{-}&{-} \\
%% Two significant units
{-}&{-}&{-}&
~~{91.32}~\scriptsize($\pm$ 0.18)$^\dagger$&~~~~{100.0}$^\dagger$&~~{-0.03}~\scriptsize($\pm$ 0.00)$^\dagger$&
{-}&{-}&{-} \\

GPM~\cite{Saha2021}&
%% One significant unit
% {95.0}~\scriptsize($\pm$ 0.1)&{$~$ 100.0}&{-0.02}~\scriptsize($\pm$ 0.01)&
% ~~{91.2}~\scriptsize($\pm$ 0.2)$^\dagger$&{$~$ 100.0}&~~{-0.01}~\scriptsize($\pm$ 0.00)$^\dagger$&
% {85.2}~\scriptsize($\pm$ 0.4)&{$~$ 100.0}&{-0.01}~\scriptsize($\pm$ 0.00) \\
%% Two significant units
{94.96}~\scriptsize($\pm$ 0.07)&{$~$ 100.0}&{-0.02}~\scriptsize($\pm$ 0.01)&
~~{91.22}~\scriptsize($\pm$ 0.20)$^\dagger$&{$~$ 100.0}&~~{-0.01}~\scriptsize($\pm$ 0.00)$^\dagger$&
{85.24}~\scriptsize($\pm$ 0.37)&{$~$ 100.0}&{-0.01}~\scriptsize($\pm$ 0.00) \\

\midrule
PackNet~\cite{mallya2018packnet}&
%% One significant unit
% {96.4}~\scriptsize($\pm$ 0.0)&{$~$ 96.4}&\textbf{0.0}&
% {92.8}~\scriptsize($\pm$ 0.1)&{$~$ 82.8}&\textbf{0.0}&
% {30.7}~\scriptsize($\pm$ 1.5)&{$~$ 399.2}&\textbf{0.0} \\
%% Two significant units
{96.37}~\scriptsize($\pm$ 0.04)&{$~$ 96.38}&\cellcolor{gg}\textbf{0.0}&
{92.81}~\scriptsize($\pm$ 0.12)&{$~$ 82.86}&\cellcolor{gg}\textbf{0.0}&
{30.70}~\scriptsize($\pm$ 1.50)&{$~$ 399.2}&\cellcolor{gg}\textbf{0.0} \\ 
\midrule
WSN, $c=0.03$&% need to add per-task sparsity
%% One significant unit
% {95.0}~\scriptsize($\pm$ 0.1)&\textbf{{$~$ 20.0}~\scriptsize($\pm$ 0.1)}&\textbf{0.0}&
% {90.6}~\scriptsize($\pm$ 0.7)&\textbf{{$~$ 12.1}~\scriptsize($\pm$ 0.1)}&\textbf{0.0}& % 8.7 + 100*(1-0.78)*5/32 = 12.1 $\pm$ 0.082
% {80.7}~\scriptsize($\pm$ 2.6)&\textbf{{$~~~$ 75.9}~\scriptsize($\pm$ 1.3)}&\textbf{0.0} \\ % 7.1 + 100*(1-0.78)*100/32 = 75.9 $\pm$ 1.24
%% Two significant unit
{94.84}~\scriptsize($\pm$ 0.11)&\textbf{{$~$ 19.87}~\scriptsize($\pm$ 0.16)}&\cellcolor{gg}\textbf{0.0}&
{90.57}~\scriptsize($\pm$ 0.65)&\textbf{{$~$ 12.11}~\scriptsize($\pm$ 0.06)}&\cellcolor{gg}\textbf{0.0}& % 8.7 + 100*(1-0.78)*5/32 = 12.1 $\pm$ 0.082
{80.68}~\scriptsize($\pm$ 2.60)&\textbf{{$~~~$ 75.87}~\scriptsize($\pm$ 1.24)}&\cellcolor{gg}\textbf{0.0} \\ % 7.1 + 100*(1-0.78)*100/32 = 75.9 $\pm$ 1.24

WSN, $c=0.05$&% need to add per-task sparsity
%% One significant unit
% {95.6}~\scriptsize($\pm$ 0.2)&{$~$ 26.3}~\scriptsize($\pm$ 0.3)&\textbf{0.0}&
% {91.6}~\scriptsize($\pm$ 0.2)&{$~$ 17.3}~\scriptsize($\pm$ 0.3)&\textbf{0.0}& % 13.8 + 100*(1-0.78)*5/32 = 17.3
% \textbf{{87.3}~\scriptsize($\pm$ 0.7)}&{$~~~$ 79.8}~\scriptsize($\pm$ 1.2)&\textbf{0.0} \\ % 11.1 + 100*(1-0.78)*100/32 = 79.8
%% Two significant units
{95.65}~\scriptsize($\pm$ 0.03)&{$~$ 26.49}~\scriptsize($\pm$ 0.16)&\cellcolor{gg}\textbf{0.0}&
{91.61}~\scriptsize($\pm$ 0.21)&{$~$ 17.26}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& % 13.8 + 100*(1-0.78)*5/32 = 17.3
\textbf{{87.28}~\scriptsize($\pm$ 0.72)}&{$~~~$ 79.85}~\scriptsize($\pm$ 1.19)&\cellcolor{gg}\textbf{0.0} \\ % 11.1 + 100*(1-0.78)*100/32 = 79.8

WSN, $c=0.1$&% need to add per-task sparsity
%% One significant unit
% {96.2}~\scriptsize($\pm$ 0.1)&{$~$ 40.7}~\scriptsize($\pm$ 0.4)&\textbf{0.0}&
% {92.7}~\scriptsize($\pm$ 0.1)&{$~$ 28.0}~\scriptsize($\pm$ 0.3)&\textbf{0.0}& % 24.6 + 100*(1-0.78)*5/32 = 28.0
% {83.1}~\scriptsize($\pm$ 1.6)&{$~~~$ 83.1}~\scriptsize($\pm$ 1.6)&\textbf{0.0} \\ % 14.3 + 100*(1-0.78)*100/32 = 83.1
%% Two significant units
{96.14}~\scriptsize($\pm$ 0.03)&{$~$ 40.41}~\scriptsize($\pm$ 0.54)&\cellcolor{gg}\textbf{0.0}&
{92.67}~\scriptsize($\pm$ 0.12)&{$~$ 28.01}~\scriptsize($\pm$ 0.28)&\cellcolor{gg}\textbf{0.0}& % 24.6 + 100*(1-0.78)*5/32 = 28.0
{83.10}~\scriptsize($\pm$ 1.56)&{$~~~$ 83.08}~\scriptsize($\pm$ 1.61)&\cellcolor{gg}\textbf{0.0} \\ % 14.3 + 100*(1-0.78)*100/32 = 83.1

WSN, $c=0.3$&% need to add per-task sparsity
%% One significant unit
% \textbf{{96.5}~\scriptsize($\pm$ 0.1)}&{$~$ 77.0}~\scriptsize($\pm$ 0.5)&{\textbf{0.0}}& % 70.2 + 100*(1-0.78)*10/32 = 73.6
% {93.2}~\scriptsize($\pm$ 0.3)&{$~$ 62.3}~\scriptsize($\pm$ 0.7)&\textbf{0.0}& % 58.9 + 100*(1-0.78)*5/32 = 62.3
% {81.9}~\scriptsize($\pm$ 1.1)&{$~$ 102.2}~\scriptsize($\pm$ 0.9)&\textbf{0.0} \\ % 33.4 + 100*(1-0.78)*100/32 = 102.2
%% Two significant units
\textbf{{96.41}~\scriptsize($\pm$ 0.07)}&{$~$ 77.73}~\scriptsize($\pm$ 0.36)&{\cellcolor{gg}\textbf{0.0}}& % 70.2 + 100*(1-0.78)*10/32 = 73.6
{93.22}~\scriptsize($\pm$ 0.32)&{$~$ 62.30}~\scriptsize($\pm$ 0.69)&\cellcolor{gg}\textbf{0.0}& % 58.9 + 100*(1-0.78)*5/32 = 62.3
{81.89}~\scriptsize($\pm$ 1.15)&{$~$ ~~102.2}~\scriptsize($\pm$ 0.89)&\cellcolor{gg}\textbf{0.0} \\ % 33.4 + 100*(1-0.78)*100/32 = 102.2

WSN, $c=0.5$&% need to add per-task sparsity
%% One significant unit
% {96.3}~\scriptsize($\pm$ 0.1)&{$~$ 97.8}~\scriptsize($\pm$ 0.3)&\textbf{0.0}& 
% \textbf{{93.4}~\scriptsize($\pm$ 0.1)}&{$~$ 86.1}~\scriptsize($\pm$ 0.6)&\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
% {79.8}~\scriptsize($\pm$ 2.2)&{$~$ 121.2}~\scriptsize($\pm$ 0.5)&\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2
%% Two significant units
{96.24}~\scriptsize($\pm$ 0.11)&{$~$ 98.10}~\scriptsize($\pm$ 0.25)&\cellcolor{gg}\textbf{0.0}& 
\textbf{{93.41}~\scriptsize($\pm$ 0.13)}&{$~$ 86.10}~\scriptsize($\pm$ 0.57)&\cellcolor{gg}\textbf{0.0}& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{79.80}~\scriptsize($\pm$ 2.16)&{$~$ ~~121.2}~\scriptsize($\pm$ 0.50)&\cellcolor{gg}\textbf{0.0} \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2


\midrule
MTL&
~~{96.70~\scriptsize($\pm$ 0.02)$^\dagger$}&~~{100.0}&{-}&
~~{91.54~\scriptsize($\pm$ 0.28)$^\dagger$}&~~{100.0}&{-}&
{81.23~\scriptsize($\pm$ 0.52)}&~~{100.0}&{-} \\
\bottomrule
\end{tabular}}
%\end{adjustbox}
\label{tab:main_table_new}
\vspace{-0.2in}
\end{center}
\end{table*}




==> materials/9_backup/5_main_table_new.tex <==
\begin{table*}[ht]
\small
\begin{center}
\caption{\small Performance comparison of the proposed method and other baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (ACC), average capacity (CAP), and average backward transfer (BWT) across $5$ independent runs. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Values with $\dagger$ and * denote reported performances from \citet{Saha2021} and \citet{Yoon2020}. PackNet~\cite{mallya2018packnet} is set to baseline as a non-reused weight model.}

%\begin{adjustbox}{width=1.0\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Method}}&\multicolumn{3}{c}{\textbf{Permuted MNIST}}&
% \multicolumn{3}{c}{\textbf{Split CIFAR-100}}&
% \multicolumn{3}{c}{\textbf{Split CIFAR-100 Superclass}}&
\multicolumn{3}{c}{\textbf{5 Datasets}}&
\multicolumn{3}{c}{\textbf{Omniglot Rotation}} \\


\midrule
&CF&
ACC (\%)&CAP (\%)&BWT&
% ACC (\%)&CAP (\%)&BWT (\%)&
% ACC (\%)&CAP (\%)&BWT (\%)&
ACC (\%)&CAP (\%)&BWT&
ACC (\%)&CAP (\%)&BWT \\
\midrule
STL&$\bsy\times$&
% {97.6}~\scriptsize($\pm$ 0.10)&{1000.0} \%&&
% {70.9}~\scriptsize($\pm$ 0.38)&{1000.0} \%&&
% {90.7}~\scriptsize($\pm$ 0.53)&{500.0} \%&&
%&&&
%&&\\
{97.2}~\scriptsize($\pm$ 0.11)&{$~$ 1000.0}~\scriptsize($\pm$ 0.00)&-&
% {73.9}~\scriptsize($\pm$ 0.44)&{$~$ 1000}~\scriptsize($\pm$ 0.00)&{0.00}~\scriptsize($\pm$ 0.00)&
% {62.0}~\scriptsize($\pm$ 0.44)&{$~$ 2000}~\scriptsize($\pm$ 0.00)&{0.00}~\scriptsize($\pm$ 0.00)&
{93.4}~\scriptsize($\pm$ 0.12)&{$~$ 500.0}~\scriptsize($\pm$ 0.00)&-&
{82.1}~\scriptsize($\pm$ 0.08){\scriptsize*}&{$~$ 10000.0}~\scriptsize($\pm$ 0.00)& - \\
 \midrule
FINETUNE&\checkmark&
% {62.5}~\scriptsize($\pm$ 2.96)&{100.0} \%&&
% {13.2}~\scriptsize($\pm$ 0.54)&{100.0} \%&&
% {36.8}~\scriptsize($\pm$ 2.25)&{100.0} \%&&
%&&&
%&&\\
~{78.2}~\scriptsize($\pm$ 0.84)&{$~$ 100.0}~\scriptsize($\pm$ 0.00)&~~{-0.21}~\scriptsize($\pm$ 0.01)&
% {17.3}~\scriptsize($\pm$ 0.28)&{$~$ 100}~\scriptsize($\pm$ 0.00)&{-65.0}~\scriptsize($\pm$ 0.40)&
% {20.0}~\scriptsize($\pm$ 0.00)&{$~$ 100}~\scriptsize($\pm$ 0.00)&{-15.3}~\scriptsize($\pm$ 5.26)&
{80.1}~\scriptsize($\pm$ 0.74)&{$~$ 100.0}~\scriptsize($\pm$ 0.00)&{-0.17}~\scriptsize($\pm$ 0.01)&
{44.5}~\scriptsize($\pm$ 1.68)&{$~$ 100.0}~\scriptsize($\pm$ 0.00)&{-0.45}~\scriptsize($\pm$ 0.02) \\


EWC~\cite{Kirkpatrick2017}&\checkmark&~{92.0}~\scriptsize($\pm$ 0.60)&~~{100.0}~\scriptsize($\pm$ 0.00)&~{-0.03}~\scriptsize($\pm$ 0.00)&
% {xx.x}~\scriptsize($\pm$ x.xx)&{x.xx} \%&{-}~\scriptsize($\pm$ -)&
% {xx.x}~\scriptsize($\pm$ x.xx)&{x.xx} \%&{-}~\scriptsize($\pm$ -)&
~~{88.6}~\scriptsize($\pm$ 0.26)$^\dagger$&~~~~{100.0}~\scriptsize($\pm$ 0.00)$^\dagger$&~~{-0.04}~\scriptsize($\pm$ 0.01)$^\dagger$&~~{68.7}~\scriptsize($\pm$ 1.92){\scriptsize*}&~~~~{100.0}~\scriptsize($\pm$ 0.00){\scriptsize*}&{-} \\




HAT~\cite{Serra2018}&\checkmark&
% {-}&{-}&&
% {72.0} $^\dagger$&{100.0} \%&&
% {88.6} $^\dagger$&{100.0} \%&&
%&&&
%&&\\
{-}&{-}&{-}&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
~~{91.3}~\scriptsize($\pm$ 0.18)$^\dagger$&~~~~{100.0}~\scriptsize($\pm$ 0.00)$^\dagger$&~~{-0.03}~\scriptsize($\pm$ 0.00)$^\dagger$&
{-}&{-}&{-} \\
% APD~\cite{Yoon2020}&\checkmark&
% {xx.x}~\scriptsize($\pm$ x.xx)&{x.xx} \%&{-}~\scriptsize($\pm$ -)&
% % {xx.x}~\scriptsize($\pm$ x.xx)&{x.xx} \%&{-}~\scriptsize($\pm$ -)&
% % {xx.x}~\scriptsize($\pm$ x.xx)&{x.xx} \%&{-}~\scriptsize($\pm$ -)&
% {xx.x}~\scriptsize($\pm$ x.xx)&{x.xx} \%&{-}~\scriptsize($\pm$ -)&
% {81.2}~\scriptsize($\pm$ 0.53) {*}&{943}~\scriptsize($\pm$ 0.00)&{-}~\scriptsize($\pm$ -) \\



% AGS-CL~\cite{Jung2020}&\checkmark&
% % {91.1}~\scriptsize($\pm$ 0.71)&{100.0} \%&&
% % {49.6}~\scriptsize($\pm$ 1.89)&{100.0} \%&&
% % {-}&-&&
% %&&&
% %&&\\
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% % {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% % {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -) \\
GPM~\cite{Saha2021}&\checkmark&
% {92.9}~\scriptsize($\pm$ 0.20)&{x.xx} \%&
% {93.9} $^\dagger$&{100.0} \%&&
% {72.5} $^\dagger$&{100.0} \%&&
% {91.3} $^\dagger$&{100.0} \%&&
%&&&
%&&\\
{95.0}~\scriptsize($\pm$ 0.07)&{$~$ 100.0}~\scriptsize($\pm$ 0.00)&{-0.02}~\scriptsize($\pm$ 0.01)&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
~~{91.2}~\scriptsize($\pm$ 0.20)$^\dagger$&{$~$ 100.0}~\scriptsize($\pm$ 0.00)&~~{-0.01}~\scriptsize($\pm$ 0.00)$^\dagger$&
{85.24}~\scriptsize($\pm$ 0.38)&{$~$ 100.0}~\scriptsize($\pm$ 0.00) &{0.01}~\scriptsize($\pm$ 0.00) \\
\midrule
PackNet~\cite{mallya2018packnet}&$\bsy\times$&
%\textbf{{95.9}~\scriptsize($\pm$ 0.05)}&{$~$ 96.8} \%&% 0.655 + 10*1/32
% {94.5}~\scriptsize($\pm$ 0.05)&{$~$ 72.1} \%&&% 0.408 + 10*1/32
% {58.3}~\scriptsize($\pm$ 0.46)&{131.2} \%&&% 0.999 + 10*1/32
% {89.0}~\scriptsize($\pm$ 0.21)&{115.4} \%&&% 0.998 + 5 * 1/32 
%&&&
%&&\\ 
{95.5}~\scriptsize($\pm$ 1.29)&{$~$ 125.6}~\scriptsize($\pm$ 0.00)&{0.00}~\scriptsize($\pm$ 0.00)&% 0.9437 + 10*1/32 % plus per-task mask
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
% {-}~\scriptsize($\pm$ -)&\textbf{{$~$ -}} \%&{-}~\scriptsize($\pm$ -)&
{92.8}~\scriptsize($\pm$ 0.12)&{$~$ 82.8}~\scriptsize($\pm$ 0.00)&{0.00}~\scriptsize($\pm$ 0.00)& % 67.2 + 100*5/32 = 82.8
% 67.2 + 100*5/32*(1-0.78) = 70.7
% {23.8}~\scriptsize($\pm$ 1.11)&{$~$ 375.9}~\scriptsize($\pm$ 0.00)&{0.00}~\scriptsize($\pm$ 0.00) \\ % 63.4 + 100*100/32 = 375.9
{30.7}~\scriptsize($\pm$ 1.50)&{$~$ 399.2}~\scriptsize($\pm$ 0.00)&{0.00}~\scriptsize($\pm$ 0.00) \\ % 86.74 + 100*100/32 = 399.2
% 86.74 + 100*100*(1-0.78)/32 = 155.5
% LL-Ticket~\cite{longliveticket}&$\bsy\times$&
% {xx.x}~\scriptsize($\pm$ x.xx)&{$~$ x.xx} \%&
% {xx.x}~\scriptsize($\pm$ x.xx)&{$~$ x.xx} \%&
% {xx.x}~\scriptsize($\pm$ x.xx)&{$~$ x.xx} \%\\
\midrule
WSN, $c=0.03$&$\bsy\times$&% need to add per-task sparsity
{95.0}~\scriptsize($\pm$ 0.11)&\textbf{{$~$ 16.6}~\scriptsize($\pm$ 0.06)}&{0.00}~\scriptsize($\pm$ 0.00)&% 13.1 + 100*(1-0.78)*10/32 = 16.57 $\pm$ 0.06
% {71.0}~\scriptsize($\pm$ 0.56)&\textbf{{$~$ 11.7}~\scriptsize($\pm$ 0.25)}&{0.00}~\scriptsize($\pm$ 0.00)&
% {62.5}~\scriptsize($\pm$ 0.40)&\textbf{{$~$ 10.4}~\scriptsize($\pm$ 0.24)}&{0.00}~\scriptsize($\pm$ 0.00)&
%{90.6}~\scriptsize($\pm$ 0.65)&\textbf{{$~$ 8.67}~\scriptsize($\pm$ 0.06)}&{0.00}~\scriptsize($\pm$ 0.00)&
{90.6}~\scriptsize($\pm$ 0.65)&\textbf{{$~$ 12.1}~\scriptsize($\pm$ 0.06)}&{0.00}~\scriptsize($\pm$ 0.00)& % 8.7 + 100*(1-0.78)*5/32 = 12.1 $\pm$ 0.082
{80.7}~\scriptsize($\pm$ 2.60)&\textbf{{$~~~$ 75.9}~\scriptsize($\pm$ 1.24)}&{0.00}~\scriptsize($\pm$ 0.00) \\ % 7.1 + 100*(1-0.78)*100/32 = 75.9 $\pm$ 1.24

WSN, $c=0.05$&$\bsy\times$&% need to add per-task sparsity
{95.6}~\scriptsize($\pm$ 0.15)&{$~$ 22.9}~\scriptsize($\pm$ 0.33)&{0.00}~\scriptsize($\pm$ 0.00)& % 19.5 + 100*(1-0.78)*10/32 = 22.9
% {72.4}~\scriptsize($\pm$ 0.44)&{$~$ 18.3}~\scriptsize($\pm$ 0.54)&{0.00}~\scriptsize($\pm$ 0.00)&
% {63.1}~\scriptsize($\pm$ 0.16)&{$~$ 14.9}~\scriptsize($\pm$ 0.63)&{0.00}~\scriptsize($\pm$ 0.00)&
{91.6}~\scriptsize($\pm$ 0.21)&{$~$ 17.3}~\scriptsize($\pm$ 0.25)&{0.00}~\scriptsize($\pm$ 0.00)& % 13.8 + 100*(1-0.78)*5/32 = 17.3
\textbf{{87.3}~\scriptsize($\pm$ 0.72)}&{$~~~$ 79.8}~\scriptsize($\pm$ 1.19)&{0.00}~\scriptsize($\pm$ 0.00) \\ % 11.1 + 100*(1-0.78)*100/32 = 79.8

WSN, $c=0.1$&$\bsy\times$&% need to add per-task sparsity
{96.2}~\scriptsize($\pm$ 0.10)&{$~$ 37.2}~\scriptsize($\pm$ 0.44)&{0.00}~\scriptsize($\pm$ 0.00)& % 33.8 + 100*(1-0.78)*10/32 = 37.2
% {74.7}~\scriptsize($\pm$ 0.33)&{$~$ 32.7}~\scriptsize($\pm$ 0.75)&{0.00}~\scriptsize($\pm$ 0.00)&
% \textbf{{63.7}~\scriptsize($\pm$ 0.39)}&{$~$ 22.9}~\scriptsize($\pm$ 1.56)&\textbf{{0.00}~\scriptsize($\pm$ 0.00)}&
{92.7}~\scriptsize($\pm$ 0.12)&{$~$ 28.0}~\scriptsize($\pm$ 0.28)&{0.00}~\scriptsize($\pm$ 0.00)& % 24.6 + 100*(1-0.78)*5/32 = 28.0
{83.1}~\scriptsize($\pm$ 1.56)&{$~~~$ 83.1}~\scriptsize($\pm$ 1.61)&{0.00}~\scriptsize($\pm$ 0.00) \\ % 14.3 + 100*(1-0.78)*100/32 = 83.1

WSN, $c=0.3$&$\bsy\times$&% need to add per-task sparsity
\textbf{{96.5}~\scriptsize($\pm$ 0.06)}&{$~$ 73.6}~\scriptsize($\pm$ 0.50)&\textbf{{0.00}~\scriptsize($\pm$ 0.00)}& % 70.2 + 100*(1-0.78)*10/32 = 73.6
% {76.4}~\scriptsize($\pm$ 0.38)&{$~$ 73.1}~\scriptsize($\pm$ 0.81)&{0.00}~\scriptsize($\pm$ 0.00)&
% {63.4}~\scriptsize($\pm$ 0.26)&{$~$ 38.2}~\scriptsize($\pm$ 0.74)&{0.00}~\scriptsize($\pm$ 0.00)&
{93.2}~\scriptsize($\pm$ 0.32)&{$~$ 62.3}~\scriptsize($\pm$ 0.69)&{0.00}~\scriptsize($\pm$ 0.00)& % 58.9 + 100*(1-0.78)*5/32 = 62.3
{81.9}~\scriptsize($\pm$ 1.14)&{$~$ 102.2}~\scriptsize($\pm$ 0.89)&{0.00}~\scriptsize($\pm$ 0.00) \\ % 33.4 + 100*(1-0.78)*100/32 = 102.2

WSN, $c=0.5$&$\bsy\times$&% need to add per-task sparsity
{96.3}~\scriptsize($\pm$ 0.08)&{$~$ 94.3}~\scriptsize($\pm$ 0.31)&{0.00}~\scriptsize($\pm$ 0.00)& % 90.9 + 100*(1-0.78)*10/32 = 94.3
% \textbf{{76.5}~\scriptsize($\pm$ 0.39)}&{$~$ 92.2}~\scriptsize($\pm$ 0.75)&\textbf{{0.00}~\scriptsize($\pm$ 0.00)}&
% {63.4}~\scriptsize($\pm$ 0.17)&{$~$ 57.0}~\scriptsize($\pm$ 0.63)&{0.00}~\scriptsize($\pm$ 0.00)&
\textbf{{93.4}~\scriptsize($\pm$ 0.13)}&{$~$ 86.1}~\scriptsize($\pm$ 0.57)&{0.00}~\scriptsize($\pm$ 0.00)& % 82.7 + 100*(1-0.78)*5/32 = 86.1
{79.8}~\scriptsize($\pm$ 2.16)&{$~$ 121.2}~\scriptsize($\pm$ 0.50)&{0.00}~\scriptsize($\pm$ 0.00) \\ % 52.4 + 100*(1-0.78)*100/32 = 121.2

% WSN, $c=0.7$&$\bsy\times$&% need to add per-task sparsity
% {96.3}~\scriptsize($\pm$ 0.08)&{$~$ 90.9}~\scriptsize($\pm$ 0.31)&{0.00}~\scriptsize($\pm$ 0.00)&
% % \textbf{{76.5}~\scriptsize($\pm$ 0.39)}&{$~$ 92.2}~\scriptsize($\pm$ 0.75)&\textbf{{0.00}~\scriptsize($\pm$ 0.00)}&
% % {63.4}~\scriptsize($\pm$ 0.17)&{$~$ 57.0}~\scriptsize($\pm$ 0.63)&{0.00}~\scriptsize($\pm$ 0.00)&
% \textbf{{93.4}~\scriptsize($\pm$ 0.13)}&{$~$ 82.7}~\scriptsize($\pm$ 0.57)&{0.00}~\scriptsize($\pm$ 0.00)&
% {79.8}~\scriptsize($\pm$ 2.16)&{$~$ 52.4}~\scriptsize($\pm$ 0.50)&{0.00}~\scriptsize($\pm$ 0.00) \\ % need to add (per-task)

% WSN, $c=0.9$&$\bsy\times$&% need to add per-task sparsity
% {96.3}~\scriptsize($\pm$ 0.08)&{$~$ 90.9}~\scriptsize($\pm$ 0.31)&{0.00}~\scriptsize($\pm$ 0.00)&
% % \textbf{{76.5}~\scriptsize($\pm$ 0.39)}&{$~$ 92.2}~\scriptsize($\pm$ 0.75)&\textbf{{0.00}~\scriptsize($\pm$ 0.00)}&
% % {63.4}~\scriptsize($\pm$ 0.17)&{$~$ 57.0}~\scriptsize($\pm$ 0.63)&{0.00}~\scriptsize($\pm$ 0.00)&
% \textbf{{93.4}~\scriptsize($\pm$ 0.13)}&{$~$ 82.7}~\scriptsize($\pm$ 0.57)&{0.00}~\scriptsize($\pm$ 0.00)&
% {79.8}~\scriptsize($\pm$ 2.16)&{$~$ 52.4}~\scriptsize($\pm$ 0.50)&{0.00}~\scriptsize($\pm$ 0.00) \\ % need to add (per-task)

\midrule
MTL&$\bsy\times$&
~~{96.7~\scriptsize($\pm$ 0.02)$^\dagger$}&{100.0}&{-}&
% {79.6 $^\dagger$}&{100.0} \%&{-}&
~~{91.5~\scriptsize($\pm$ 0.28)$^\dagger$}&{100.0}&{-}&
% {-}&{-} \%&{-}&
{81.2~\scriptsize($\pm$ 0.50)}&{100.0}&{-} \\
\bottomrule
\end{tabular}}
%\end{adjustbox}
\label{tab:main_table_new}
\end{center}
\end{table*}




==> materials/9_backup/5_main_table_sota.tex <==
\begin{table*}[t]
\small
\begin{center}
\caption{\small  Performance comparisons of the proposed method and other state-of-the-art on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (ACC), average capacity (CAP), and average backward transfer (BWT) across $5$ independent runs with 5 seeds under the same experimental setup \cite{deng2021flattening}. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Also, $\dagger$ $~$ denotes results reported from \cite{deng2021flattening}.}

\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular}{l|c|ccc|ccc|ccccc}
\toprule
\multicolumn{2}{c}{\textbf{Method}}&\multicolumn{3}{c}{\textbf{CIFAR-100 Split}} & \multicolumn{3}{c}{\textbf{CIFAR-100 Superclass}} & \multicolumn{3}{c}{\textbf{TinyImageNet}} \\


\midrule
& CF & ACC (\%) & CAP (\%) & BWT (\%) & ACC (\%) & CAP (\%) & BWT (\%) & ACC (\%) & CAP (\%) & BWT (\%)  \\
\midrule
La-MaML \cite{gupta2020maml} & \checkmark  & 71.37~\scriptsize($\pm$ 0.67)$^\dagger$ & 100.0 & -5.39~\scriptsize($\pm$ 0.53)$^\dagger$ & 54.44~\scriptsize($\pm$ 1.36)$^\dagger$ & 100.0  & -6.65~\scriptsize($\pm$ 0.85)$^\dagger$ & 66.90~\scriptsize($\pm$ 1.65)$^\dagger$ & 100.0  & -9.13~\scriptsize($\pm$ 0.90)$^\dagger$  \\
GPM \cite{Saha2021} & \checkmark   & 73.18~\scriptsize($\pm$ 0.52)$^\dagger$ & 100.0 & -1.17~\scriptsize($\pm$ 0.27)$^\dagger$ & 57.33~\scriptsize($\pm$ 0.37)$^\dagger$ & 100.0  & -0.37~\scriptsize($\pm$ 0.12)$^\dagger$ & 67.39~\scriptsize($\pm$ 0.47)$^\dagger$ & 100.0  & ~\textbf{1.45}~\scriptsize($\pm$ \textbf{0.22})$^\dagger$  \\
FS-DGPM \cite{deng2021flattening} & \checkmark  & 74.33~\scriptsize($\pm$ 0.31)$^\dagger$ & 100.0 & -2.17~\scriptsize($\pm$ 0.17)$^\dagger$ & 58.81~\scriptsize($\pm$ 0.34)$^\dagger$  & 100.0  & -2.97~\scriptsize($\pm$ 0.35)$^\dagger$ & 70.41~\scriptsize($\pm$ 1.30)$^\dagger$  & 100.0  & -2.11~\scriptsize($\pm$ 0.84)$^\dagger$ \\

\midrule

%WSN, $c=0.03$ & $\bsy \times$ & 70.65~\scriptsize($\pm$ 0.36) & \textbf{11.69}~\scriptsize($\pm$ \textbf{0.25}) & 0.0~\scriptsize($\pm$ 0.0) & 54.99~\scriptsize($\pm$ 0.71) & ~~\textbf{8.55}~\scriptsize($\pm$ \textbf{0.22})  & 0.0~\scriptsize($\pm$ 0.0) & 68.72~\scriptsize($\pm$ 1.63) & ~~\textbf{9.69}~\scriptsize($\pm$ \textbf{0.21})  & 0.0~\scriptsize($\pm$ 0.0)  \\
WSN, $c=0.03$ & $\bsy \times$ & 70.65~\scriptsize($\pm$ 0.36) & \textbf{18.56}~\scriptsize($\pm$ \textbf{0.25}) & 0.0~\scriptsize($\pm$ 0.0) & 54.99~\scriptsize($\pm$ 0.71) & \textbf{22.30}~\scriptsize($\pm$ \textbf{0.22})  & 0.0~\scriptsize($\pm$ 0.0) & 68.72~\scriptsize($\pm$ 1.63) & \textbf{37.19}~\scriptsize($\pm$ \textbf{0.21})  & 0.0~\scriptsize($\pm$ 0.0)  \\

%WSN, $c=0.05$ & $\bsy \times$ & 72.44~\scriptsize($\pm$ 0.27) & 18.22~\scriptsize($\pm$ 0.42) & 0.0~\scriptsize($\pm$ 0.0) & 57.99~\scriptsize($\pm$ 1.34) & 13.62~\scriptsize($\pm$ 0.33)  & 0.0~\scriptsize($\pm$ 0.0) & 71.22~\scriptsize($\pm$ 0.94) & 14.48~\scriptsize($\pm$ 0.52)  & 0.0~\scriptsize($\pm$ 0.0)  \\
WSN, $c=0.05$ & $\bsy \times$ & 72.44~\scriptsize($\pm$ 0.27) & 25.09~\scriptsize($\pm$ 0.42) & 0.0~\scriptsize($\pm$ 0.0) & 57.99~\scriptsize($\pm$ 1.34) & 27.37~\scriptsize($\pm$ 0.33)  & 0.0~\scriptsize($\pm$ 0.0) & 71.22~\scriptsize($\pm$ 0.94) & 41.98~\scriptsize($\pm$ 0.52)  & 0.0~\scriptsize($\pm$ 0.0)  \\


%WSN, $c=0.1$ & $\bsy \times$ & 74.55~\scriptsize($\pm$ 0.47) & 33.00~\scriptsize($\pm$ 0.62) & 0.0~\scriptsize($\pm$ 0.0) & 60.45~\scriptsize($\pm$ 0.37) & 24.80~\scriptsize($\pm$ 0.20)  & 0.0~\scriptsize($\pm$ 0.0) & \textbf{71.96}~\scriptsize($\pm$ \textbf{1.41}) & 21.15~\scriptsize($\pm$ 3.03)  & 0.0~\scriptsize($\pm$ 0.0)  \\
WSN, $c=0.1$ & $\bsy \times$ & 74.55~\scriptsize($\pm$ 0.47) & 39.87~\scriptsize($\pm$ 0.62) & 0.0~\scriptsize($\pm$ 0.0) & 60.45~\scriptsize($\pm$ 0.37) & 38.55~\scriptsize($\pm$ 0.20)  & 0.0~\scriptsize($\pm$ 0.0) & \textbf{71.96}~\scriptsize($\pm$ \textbf{1.41}) & 48.65~\scriptsize($\pm$ 3.03)  & 0.0~\scriptsize($\pm$ 0.0)  \\

%WSN, $c=0.3$ & $\bsy \times$ & 75.98~\scriptsize($\pm$ 0.68) & 73.39~\scriptsize($\pm$ 1.53) & 0.0~\scriptsize($\pm$ 0.0) & 61.47~\scriptsize($\pm$ 0.30) & 49.72~\scriptsize($\pm$ 1.33) & 0.0~\scriptsize($\pm$ 0.0) & 70.92~\scriptsize($\pm$ 1.37) & 45.94~\scriptsize($\pm$ 2.35)  & 0.0~\scriptsize($\pm$ 0.0)  \\
WSN, $c=0.3$ & $\bsy \times$ & 75.98~\scriptsize($\pm$ 0.68) & 80.26~\scriptsize($\pm$ 1.53) & 0.0~\scriptsize($\pm$ 0.0) & 61.47~\scriptsize($\pm$ 0.30) & 63.47~\scriptsize($\pm$ 1.33) & 0.0~\scriptsize($\pm$ 0.0) & 70.92~\scriptsize($\pm$ 1.37) & 73.44~\scriptsize($\pm$ 2.35)  & 0.0~\scriptsize($\pm$ 0.0)  \\


%WSN, $c=0.5$ & $\bsy \times$ & 76.38~\scriptsize($\pm$ 0.34) & 92.26~\scriptsize($\pm$ 0.48) & 0.0~\scriptsize($\pm$ 0.0) & \textbf{61.79}~\scriptsize($\pm$ \textbf{0.23}) & 67.18~\scriptsize($\pm$ 1.58) & \textbf{0.0}~\scriptsize($\pm$ \textbf{0.0}) & 69.06~\scriptsize($\pm$ 0.82) & 64.53~\scriptsize($\pm$ 1.80)  & 0.0~\scriptsize($\pm$ 0.0)  \\
WSN, $c=0.5$ & $\bsy \times$ & \textbf{76.38}~\scriptsize($\pm$ \textbf{0.34}) & 99.13~\scriptsize($\pm$ 0.48) & 0.0~\scriptsize($\pm$ 0.0) & \textbf{61.79}~\scriptsize($\pm$ \textbf{0.23}) & 80.93~\scriptsize($\pm$ 1.58) & \textbf{0.0}~\scriptsize($\pm$ \textbf{0.0}) & 69.06~\scriptsize($\pm$ 0.82) & 92.03~\scriptsize($\pm$ 1.80)  & 0.0~\scriptsize($\pm$ 0.0)  \\


%WSN, $c=0.7$ & $\bsy \times$ & \textbf{76.88}~\scriptsize($\pm$ \textbf{0.51}) & 98.90~\scriptsize($\pm$ 0.16) & \textbf{0.0}~\scriptsize($\pm$ \textbf{0.0}) & 61.24~\scriptsize($\pm$ 0.16) & 83.65~\scriptsize($\pm$ 1.03) & 0.0~\scriptsize($\pm$ 0.0) & 67.18~\scriptsize($\pm$ 1.62) & 81.32~\scriptsize($\pm$ 1.32)  & 0.0~\scriptsize($\pm$ 0.0)  \\
%WSN, $c=0.7$ & $\bsy \times$ & \textbf{76.88}~\scriptsize($\pm$ \textbf{0.51}) & 105.77~\scriptsize($\pm$ 0.16) & \textbf{0.0}~\scriptsize($\pm$ \textbf{0.0}) & 61.24~\scriptsize($\pm$ 0.16) & 97.40~\scriptsize($\pm$ 1.03) & 0.0~\scriptsize($\pm$ 0.0) & 67.18~\scriptsize($\pm$ 1.62) & 108.82~\scriptsize($\pm$ 1.32)  & 0.0~\scriptsize($\pm$ 0.0)  \\

%WSN, $c=0.9$ & $\bsy \times$ & 75.04~\scriptsize($\pm$ 0.52) & 99.98~\scriptsize($\pm$ 0.01) & 0.0~\scriptsize($\pm$ 0.0) & 58.16~\scriptsize($\pm$ 0.56) & 96.78~\scriptsize($\pm$ 0.39) & 0.0~\scriptsize($\pm$ 0.0) & 60.75~\scriptsize($\pm$ 1.02) & 94.25~\scriptsize($\pm$ 0.54)  & 0.0~\scriptsize($\pm$ 0.0)  \\
%WSN, $c=0.9$ & $\bsy \times$ & 75.04~\scriptsize($\pm$ 0.52) & 106.85~\scriptsize($\pm$ 0.01) & 0.0~\scriptsize($\pm$ 0.0) & 58.16~\scriptsize($\pm$ 0.56) & 110.53~\scriptsize($\pm$ 0.39) & 0.0~\scriptsize($\pm$ 0.0) & 60.75~\scriptsize($\pm$ 1.02) & 121.75~\scriptsize($\pm$ 0.54)  & 0.0~\scriptsize($\pm$ 0.0)  \\

\midrule

Multitask & $\bsy \times$ & 79.75~\scriptsize($\pm$ 0.38)$^\dagger$ & 100.0 & - & 61.00~\scriptsize($\pm$ 0.20)$^\dagger$ & 100.0  & - & 77.10~\scriptsize($\pm$ 1.06)$^\dagger$ & 100.0  & - \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main_sota_table}
\end{center}
\end{table*}


==> materials/9_backup/5_main_table_sota_full.tex <==
\begin{table*}[ht]
\vspace{-0.1in}
\small
\begin{center}
\caption{\small  Performance comparisons of the proposed method and other state-of-the-art on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (ACC), average capacity (CAP), and average backward transfer (BWT) across $5$ independent runs with 5 seeds under the same experimental setup \cite{deng2021flattening}. The best results are highlighted in bold. Also, $\dagger$ $~$ and $\ast$ denotes results reported from \cite{deng2021flattening} and \cite{gupta2020maml} respectively.}

\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}}&\multicolumn{3}{c}{\textbf{CIFAR-100 Split}}&
\multicolumn{3}{c}{\textbf{CIFAR-100 Superclass}}&
\multicolumn{3}{c}{\textbf{TinyImageNet}} \\

\midrule
&ACC (\%)&CAP (\%)&BWT (\%)&
ACC (\%)&CAP (\%)&BWT (\%)&
ACC (\%)&CAP (\%)&BWT (\%) \\
\midrule


EWC \cite{Kirkpatrick2017} & 72.77~\scriptsize($\pm$ 0.45)$^\dagger$ & 100.0 & ~~-3.59~\scriptsize($\pm$ 0.55)$^\dagger$ & 50.26~\scriptsize($\pm$ 1.48)$^\dagger$ & 100.0  & ~~-7.87~\scriptsize($\pm$ 1.63)$^\dagger$ & - & - & -  \\

GEM \cite{Lopez-Paz2017} & 70.15~\scriptsize($\pm$ 0.34)$^\dagger$ & 100.0 & ~~-8.61~\scriptsize($\pm$ 0.42)$^\dagger$ & 50.35~\scriptsize($\pm$ 0.80)$^\dagger$ & 100.0  & ~~-9.50~\scriptsize($\pm$ 0.85)$^\dagger$ & 50.57~\scriptsize($\pm$ 0.61)$^\ast$ & 100.0 & -20.50~\scriptsize($\pm$ 0.10)$^\ast$  \\

ICARL \cite{rebuffi2017icarl} & 53.50~\scriptsize($\pm$ 0.81)$^\dagger$ & 100.0 & -20.44~\scriptsize($\pm$ 0.82)$^\dagger$ & 49.05~\scriptsize($\pm$ 0.51)$^\dagger$ & 100.0  & -11.24~\scriptsize($\pm$ 0.27)$^\dagger$ & 54.77~\scriptsize($\pm$ 0.32)$^\ast$ & 100.0 & ~~-3.93~\scriptsize($\pm$ 0.55)$^\ast$  \\

ER \cite{chaudhry2019continual} & 70.07~\scriptsize($\pm$ 0.35)$^\dagger$ & 100.0 & ~~-7.70~\scriptsize($\pm$ 0.59)$^\dagger$ & 51.64~\scriptsize($\pm$ 1.09)$^\dagger$ & 100.0  & ~~-7.86~\scriptsize($\pm$ 0.89)$^\dagger$ & 48.32~\scriptsize($\pm$ 1.51)$^\ast$ & 100.0 & -19.86~\scriptsize($\pm$ 0.70)$^\ast$  \\


La-MaML \cite{gupta2020maml} & 71.37~\scriptsize($\pm$ 0.67)$^\dagger$ & 100.0 & ~~-5.39~\scriptsize($\pm$ 0.53)$^\dagger$ & 54.44~\scriptsize($\pm$ 1.36)$^\dagger$ & 100.0  & ~~-6.65~\scriptsize($\pm$ 0.85)$^\dagger$ & 66.90~\scriptsize($\pm$ 1.65)$^\dagger$ & 100.0  & ~~-9.13~\scriptsize($\pm$ 0.90)$^\dagger$  \\
GPM \cite{Saha2021} & 73.18~\scriptsize($\pm$ 0.52)$^\dagger$ & 100.0 & ~~-1.17~\scriptsize($\pm$ 0.27)$^\dagger$ & 57.33~\scriptsize($\pm$ 0.37)$^\dagger$ & 100.0  & ~~-0.37~\scriptsize($\pm$ 0.12)$^\dagger$ & 67.39~\scriptsize($\pm$ 0.47)$^\dagger$ & 100.0  & ~~~\textbf{1.45~\scriptsize($\pm$ 0.22)}$^\dagger$  \\
FS-DGPM \cite{deng2021flattening} & 74.33~\scriptsize($\pm$ 0.31)$^\dagger$ & 100.0 & ~~-2.71~\scriptsize($\pm$ 0.17)$^\dagger$ & 58.81~\scriptsize($\pm$ 0.34)$^\dagger$  & 100.0  & ~~-2.97~\scriptsize($\pm$ 0.35)$^\dagger$ & 70.41~\scriptsize($\pm$ 1.30)$^\dagger$  & 100.0  & ~~-2.11~\scriptsize($\pm$ 0.84)$^\dagger$ \\
\midrule

WSN, $c=0.03$ & 70.65~\scriptsize($\pm$ 0.36) & \textbf{18.56}~\scriptsize($\pm$ \textbf{0.25}) & \cellcolor{gg}\textbf{0.0} & 54.99~\scriptsize($\pm$ 0.71) & \textbf{22.30}~\scriptsize($\pm$ \textbf{0.22})  & \cellcolor{gg}\textbf{0.0} & 68.72~\scriptsize($\pm$ 1.63) & \textbf{37.19}~\scriptsize($\pm$ \textbf{0.21})  & \cellcolor{gg}\textbf{0.0}  \\

WSN, $c=0.05$ & 72.44~\scriptsize($\pm$ 0.27) & 25.09~\scriptsize($\pm$ 0.42) & \cellcolor{gg}\textbf{0.0} & 57.99~\scriptsize($\pm$ 1.34) & 27.37~\scriptsize($\pm$ 0.33)  & \cellcolor{gg}\textbf{0.0} & 71.22~\scriptsize($\pm$ 0.94) & 41.98~\scriptsize($\pm$ 0.52)  & \cellcolor{gg}\textbf{0.0}  \\

WSN, $c=0.1$ & 74.55~\scriptsize($\pm$ 0.47) & 39.87~\scriptsize($\pm$ 0.62) & \cellcolor{gg}\textbf{0.0} & 60.45~\scriptsize($\pm$ 0.37) & 38.55~\scriptsize($\pm$ 0.20)  & \cellcolor{gg}\textbf{0.0} & \textbf{71.96}~\scriptsize($\pm$ \textbf{1.41}) & 48.65~\scriptsize($\pm$ 3.03)  & \cellcolor{gg}\textbf{0.0}  \\

WSN, $c=0.3$ & 75.98~\scriptsize($\pm$ 0.68) & 80.26~\scriptsize($\pm$ 1.53) & \cellcolor{gg}\textbf{0.0} & 61.47~\scriptsize($\pm$ 0.30) & 63.47~\scriptsize($\pm$ 1.33) & \cellcolor{gg}\textbf{0.0} & 70.92~\scriptsize($\pm$ 1.37) & 73.44~\scriptsize($\pm$ 2.35)  & \cellcolor{gg}\textbf{0.0}  \\

WSN, $c=0.5$ & \textbf{76.38}~\scriptsize($\pm$ \textbf{0.34}) & 99.13~\scriptsize($\pm$ 0.48) & \cellcolor{gg}\textbf{0.0} & \textbf{61.79}~\scriptsize($\pm$ \textbf{0.23}) & 80.93~\scriptsize($\pm$ 1.58) & \cellcolor{gg}\textbf{0.0} & 69.06~\scriptsize($\pm$ 0.82) & 92.03~\scriptsize($\pm$ 1.80)  & \cellcolor{gg}\textbf{0.0}  \\

\midrule
Multitask & ~~79.75~\scriptsize($\pm$ 0.38)$^\dagger$ & 100.0 & - & ~~61.00~\scriptsize($\pm$ 0.20)$^\dagger$ & 100.0 & - & ~~77.10~\scriptsize($\pm$ 1.06)$^\dagger$ & 100.0 & - \\
\bottomrule
\end{tabular}}
%\end{adjustbox}
\label{tab:main_sota_full_table}
\end{center}\vspace{-0.2in}
\end{table*}

==> materials/9_backup/5_main_table_sota_larger.tex <==
\begin{table*}[ht]
\vspace{-0.1in}
\small
\begin{center}
\caption{\small  Performance comparisons of the proposed method and other state-of-the-art on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (ACC), average capacity (CAP), and average backward transfer (BWT) across $5$ independent runs with 5 seeds under the same experimental setup \cite{deng2021flattening}. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Also, $\dagger$ $~$ denotes results reported from \citet{deng2021flattening}.}

\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}}&\multicolumn{3}{c}{\textbf{CIFAR-100 Split}}&
\multicolumn{3}{c}{\textbf{CIFAR-100 Superclass}}&
\multicolumn{3}{c}{\textbf{TinyImageNet}} \\

\midrule
&ACC (\%)&CAP (\%)&BWT (\%)&
ACC (\%)&CAP (\%)&BWT (\%)&
ACC (\%)&CAP (\%)&BWT (\%) \\
\midrule

La-MaML \cite{gupta2020maml} & 71.37~\scriptsize($\pm$ 0.67)$^\dagger$ & 100.0 & -5.39~\scriptsize($\pm$ 0.53)$^\dagger$ 
& 54.44~\scriptsize($\pm$ 1.36)$^\dagger$ & 100.0  & -6.65~\scriptsize($\pm$ 0.85)$^\dagger$ & 66.90~\scriptsize($\pm$ 1.65)$^\dagger$ & 100.0  & -9.13~\scriptsize($\pm$ 0.90)$^\dagger$  \\

GPM \cite{Saha2021} & 73.18~\scriptsize($\pm$ 0.52)$^\dagger$ & 100.0 & -1.17~\scriptsize($\pm$ 0.27)$^\dagger$ & 57.33~\scriptsize($\pm$ 0.37)$^\dagger$ & 100.0  & -0.37~\scriptsize($\pm$ 0.12)$^\dagger$ & 67.39~\scriptsize($\pm$ 0.47)$^\dagger$ & 100.0  & ~\textbf{1.45}~\scriptsize($\pm$ \textbf{0.22})$^\dagger$  \\

FS-DGPM \cite{deng2021flattening} & 74.33~\scriptsize($\pm$ 0.31)$^\dagger$ & 100.0 & -2.71~\scriptsize($\pm$ 0.17)$^\dagger$ & 58.81~\scriptsize($\pm$ 0.34)$^\dagger$  & 100.0  & -2.97~\scriptsize($\pm$ 0.35)$^\dagger$ & 70.41~\scriptsize($\pm$ 1.30)$^\dagger$  & 100.0  & -2.11~\scriptsize($\pm$ 0.84)$^\dagger$ \\
\midrule

WSN, $c=0.03$ & 70.65~\scriptsize($\pm$ 0.36) & \textbf{18.56}~\scriptsize($\pm$ \textbf{0.25}) & \cellcolor{gg}\textbf{0.0} & 54.99~\scriptsize($\pm$ 0.71) & \textbf{22.30}~\scriptsize($\pm$ \textbf{0.22})  & \cellcolor{gg}\textbf{0.0} & 68.72~\scriptsize($\pm$ 1.63) & \textbf{37.19}~\scriptsize($\pm$ \textbf{0.21})  & \cellcolor{gg}\textbf{0.0}  \\

WSN, $c=0.05$ & 72.44~\scriptsize($\pm$ 0.27) & 25.09~\scriptsize($\pm$ 0.42) & \cellcolor{gg}\textbf{0.0} & 57.99~\scriptsize($\pm$ 1.34) & 27.37~\scriptsize($\pm$ 0.33)  & \cellcolor{gg}\textbf{0.0} & 71.22~\scriptsize($\pm$ 0.94) & 41.98~\scriptsize($\pm$ 0.52)  & \cellcolor{gg}\textbf{0.0}  \\

WSN, $c=0.1$ & 74.55~\scriptsize($\pm$ 0.47) & 39.87~\scriptsize($\pm$ 0.62) & \cellcolor{gg}\textbf{0.0} & 60.45~\scriptsize($\pm$ 0.37) & 38.55~\scriptsize($\pm$ 0.20)  & \cellcolor{gg}\textbf{0.0} & \textbf{71.96}~\scriptsize($\pm$ \textbf{1.41}) & 48.65~\scriptsize($\pm$ 3.03)  & \cellcolor{gg}\textbf{0.0}  \\

WSN, $c=0.3$ & 75.98~\scriptsize($\pm$ 0.68) & 80.26~\scriptsize($\pm$ 1.53) & \cellcolor{gg}\textbf{0.0} & 61.47~\scriptsize($\pm$ 0.30) & 63.47~\scriptsize($\pm$ 1.33) & \cellcolor{gg}\textbf{0.0} & 70.92~\scriptsize($\pm$ 1.37) & 73.44~\scriptsize($\pm$ 2.35)  & \cellcolor{gg}\textbf{0.0}  \\

WSN, $c=0.5$ & \textbf{76.38}~\scriptsize($\pm$ \textbf{0.34}) & 99.13~\scriptsize($\pm$ 0.48) & \cellcolor{gg}\textbf{0.0} & \textbf{61.79}~\scriptsize($\pm$ \textbf{0.23}) & 80.93~\scriptsize($\pm$ 1.58) & \cellcolor{gg}\textbf{0.0} & 69.06~\scriptsize($\pm$ 0.82) & 92.03~\scriptsize($\pm$ 1.80)  & \cellcolor{gg}\textbf{0.0}  \\

\midrule
Multitask & ~~79.75~\scriptsize($\pm$ 0.38)$^\dagger$ & 100.0 & - & ~~61.00~\scriptsize($\pm$ 0.20)$^\dagger$ & 100.0 & - & ~~77.10~\scriptsize($\pm$ 1.06)$^\dagger$ & 100.0 & - \\
\bottomrule
\end{tabular}}
%\end{adjustbox}
\label{tab:main_sota_table}
\end{center}\vspace{-0.2in}
\end{table*}

==> materials/9_backup/5_per_layer_sparsity.tex <==
\begin{figure*}[ht]
    \centering
    \setlength{\tabcolsep}{-20pt}{%
    \begin{tabular}{ccc}
    \includegraphics[width=5.cm]{images/5_per_layer_sparsity_pmnist.pdf}&
    \includegraphics[width=5.cm]{images/5_per_layer_sparsity_cifar.pdf}&
    \includegraphics[width=5.cm]{images/5_per_layer_sparsity_5DATA.pdf} \\
    \multicolumn{3}{c}{(a) Layer Capacity over Increasing Number of Tasks} & 
    % \multicolumn{1}{c}{(b) SplitCIFAR100-AlexNet} &
    % \multicolumn{1}{c}{(c) Mixture-ResNet18}
    \\
    \end{tabular}}
    \caption{\footnotesize \textbf{\% used weights per layer vs \# of tasks seen}}
    \label{fig:per_layer_sparsity}
\end{figure*}

==> materials/9_backup/5_same_network_different_data.tex <==
\begin{figure*}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ccc}
    \includegraphics[height=3.cm]{figures/p1.pdf}&
    \includegraphics[height=3.cm]{figures/p2.pdf}&
    \includegraphics[height=3.cm]{figures/p3.pdf} \\
    \multicolumn{1}{c}{(a) Lower Layer} & 
    \multicolumn{1}{c}{(b) Middle Layer} &
    \multicolumn{1}{c}{(c) Higher Layer}\\
    \end{tabular}}
    \caption{\footnotesize \textbf{Same Network Different Data - Catastrophic Forgetting as Property of Data}}
    \label{fig:cf_as_data_property}
\end{figure*}

==> materials/9_backup/6_app_5datasets.tex <==
\begin{table*}[h!]
%\vspace{-0.1in}
\centering
\caption{5-Dataset Statistics. For the datasets with monochromatic images, we replicate the image across all RGB channels so that size of each image becomes $3 \times 32 \times 32$}

% \begin{adjustbox}{width=\textwidth}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{llllll}
\toprule
& \textbf{CIFAR-10} & \textbf{MNIST} & \textbf{SVHN} & \textbf{Fashion MNIST} & \textbf{notMNIST}  \\
\midrule
%Input size &  $1\times28\times28$ &  $3\times 32\times 32$ & $3\times32\times32$ &  $3\times64\times64$ & \\
%\# tasks & $20$  & $10$  & $20$  & $40$ &  \\
\# Classes  & $10$ & $10$ & $10$ & $10$ & $10$  \\
\# Training samples & $47,500$ & $57,000$  & $69,595$  & $57,000$ & $16,011$  \\
\# Validation samples & $2,500$  & $3,000$  & $3,662$  & $3,000$ & $842$  \\
\# Test samples & $10,000$  & $10,000$  & $26,032$  & $10,000$  & $1,873$ \\
\bottomrule
\end{tabular}
%}
% \end{adjustbox}
\label{tab:main_5data_table}
% \vspace{-0.2in}
\end{table*}

==> materials/9_backup/6_app_data_statistics.tex <==
\begin{table*}[h!]
%\vspace{-0.1in}
\centering
\caption{Dataset Statistics for Comparisions with NeuralPS.}

% \begin{adjustbox}{width=\textwidth}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
\toprule
& \textbf{PMNIST} & \textbf{CIFAR-100 Split} & \textbf{CIFAR-100 Superclass} & \textbf{TinyImageNet} \\
\midrule
Input size &  $1\times28\times28$ &  $3\times 32\times 32$ & $3\times32\times32$ &  $3\times64\times64$ \\
\# tasks & $20$  & $10$  & $20$  & $40$  \\
\# Classes/task & $10$ & $10$ & $5$ & $5$  \\
\# Training/task & $1,000$ & $4,750$  & $2,375$  & $2,250$  \\
\# Validation/task & $-$  & $250$  & $125$  & $250$  \\
\# Test/task & $10,000$  & $1,000$  & $500$  & $250$  \\
\bottomrule
\end{tabular}
%}
% \end{adjustbox}
\label{tab:main_data_table}
% \vspace{-0.2in}
\end{table*}

==> materials/9_backup/6_app_data_statistics_baseline.tex <==
\begin{table*}[h!]
%\vspace{-0.1in}
\centering
\caption{Dataset Statistics for Comparisions with ICML.}

% \begin{adjustbox}{width=\textwidth}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
\toprule
& \textbf{PMNIST} & \textbf{CIFAR-100 Split} & \textbf{CIFAR-100 Superclass} & \textbf{Omniplot Rotation} \\
\midrule
Input size &  $1\times28\times28$ &  $3\times 32\times 32$ & $3\times32\times32$ &  $3\times64\times64$ \\
\# tasks & $10$  & $10$  & $20$  & $40$  \\
\# Classes/task & $10$ & $10$ & $5$ & $5$  \\
\# Training/task & $54,000$ & $4,750$  & $2,375$  & $2,250$  \\
\# Validation/task & $6,000$  & $250$  & $125$  & $250$  \\
\# Test/task & $10,000$  & $1,000$  & $500$  & $250$  \\
\bottomrule
\end{tabular}
%}
% \end{adjustbox}
\label{tab:main_data_table_baseline}
% \vspace{-0.2in}
\end{table*}

==> materials/9_backup/6_app_hyper_params.tex <==
\begin{table}[h!]
\vspace{-0.1in}
\small
\centering
\caption{\small  List of hyperparameters for the baselines and our WSN. Here, 'lr' and 'optim' represents (initial) learning rate and optimizer used for training. We represent PMNIST as 'perm', 5-Datasets as '5data', Omniglot Rotation as 'omniglot', CIFAR-100 Split as 'cifar100-split', and CIFAR-100 Superclass as 'cifar100-sc'.}

% \begin{adjustbox}{width=\textwidth}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll}
\toprule
\textbf{Methods} & \textbf{Hyperparameters} \\
\midrule
EWC & lr : 0.03 (perm) \\
& optim : sgd \\
& regularization coefficient : 1000 (perm) \\
\midrule
GPM & lr : 0.01(perm, omniglot), 0.1 (5data) \\
& optim : sgd \\
& $n_s$ : 300 (perm), 100 (5data), 125 (omniglot) \\
\midrule
PackNet & lr = 0.001 (perm, 5data, omniglot) \\
& optim : adam \\
& $c$ : 0.1 (perm), 0.2 (5data), 0.02 (omniglot) \\
\midrule
WSN (ours) & lr = 0.001 \\
& (perm, 5data, omniglot, \\
& cifar100-split, cifar100-sc, tinyimagenet) \\
& optim : adam \\
\bottomrule
\end{tabular}
}
% \end{adjustbox}
\label{tab:main_hyper_table}
% \vspace{-0.2in}
\end{table}


==> materials/9_backup/6_app_main_table.tex <==
\begin{table*}[t]
\tiny
\begin{center}
\caption{\small Performance comparison of the proposed method and other baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (Accuracy) and average forgetting (Forgetting) across $5$ independent runs. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Values with $\dagger$ $~$ denote reported performances from \cite{Saha2021}. PackNet~\cite{mallya2018packnet} is baseline.}

\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Method}}&\multicolumn{2}{c}{\textbf{Permuted MNIST}} & \multicolumn{2}{c}{\textbf{Split CIFAR-100}} & \multicolumn{2}{c}{\textbf{5 Datasets}} \\


\midrule
& CF & Accuracy & Capacity Used & Accuracy & Capacity Used & Accuracy & Capacity Used\\
\midrule
STL & $\bsy\times$ &
{\scriptsize 97.6} ($\pm$ 0.10) & {\scriptsize 1000.0} \%&
{\scriptsize 70.9} ($\pm$ 0.38) & {\scriptsize 1000.0} \%&
{\scriptsize 90.7} ($\pm$ 0.53) & {\scriptsize 500.0} \%\\
 \midrule
FINETUNE&  \checkmark &
{\scriptsize 62.5} ($\pm$ 2.96) & {\scriptsize 100.0} \%&
{\scriptsize 13.2} ($\pm$ 0.54) & {\scriptsize 100.0} \%&
{\scriptsize 36.8} ($\pm$ 2.25) & {\scriptsize 100.0} \%\\
HAT~\cite{Serra2018} &  \checkmark &
{\scriptsize -}  & {\scriptsize -} &
{\scriptsize 72.0} $\dagger$ & {\scriptsize 100.0} \%&
{\scriptsize 88.6} $\dagger$ & {\scriptsize 100.0} \%\\
% APD~\cite{Yoon2020}  & \checkmark &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%\\

AGS-CL~\cite{Jung2020} & \checkmark &
{\scriptsize 91.1} ($\pm$ 0.71) & {\scriptsize 100.0} \%&
{\scriptsize 49.6} ($\pm$ 1.89) & {\scriptsize 100.0} \%&
{\scriptsize -}  & -\\

GPM~\cite{Saha2021} & \checkmark &
% {\scriptsize 92.9} ($\pm$ 0.20) & {\scriptsize x.xx} \%&
{\scriptsize 93.9} $\dagger$ & {\scriptsize 100.0} \%&
{\scriptsize 72.5} $\dagger$ & {\scriptsize 100.0} \%&
{\scriptsize 91.3} $\dagger$ & {\scriptsize 100.0} \%\\
\cmidrule{1-8}
PackNet~\cite{mallya2018packnet}  & $\bsy\times$ &
%\textbf{{\scriptsize 95.9} ($\pm$ 0.05)} & {\scriptsize $~$ 96.8} \%& % 0.655 + 10*1/32
{\scriptsize 94.5} ($\pm$ 0.05) & {\scriptsize $~$ 72.1} \%& % 0.408 + 10*1/32
{\scriptsize 58.3} ($\pm$ 0.46) & {\scriptsize 131.2} \%& % 0.999 + 10*1/32
{\scriptsize 89.0} ($\pm$ 0.21) & {\scriptsize 115.4} \%\\ % 0.998 + 5 * 1/32
% LL-Ticket~\cite{longliveticket}  & $\bsy\times$ &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%\\
\cmidrule{1-8}
CST (Ours, SGD) $c=0.03$ & $\bsy\times$ &
{\scriptsize .} ($\pm$ 0.06) & \textbf{{\scriptsize $~$ 37.4}} \%&
{\scriptsize .} ($\pm$ 0.63) & \textbf{{\scriptsize $~$ 39.4}} \%&
{\scriptsize .} ($\pm$ 0.10) & \textbf{{\scriptsize $~$ 24.2}} \%\\
CST (Ours, SGD) $c=0.1$ & $\bsy\times$ &
{\scriptsize .} ($\pm$ 0.09) & {\scriptsize $~$ 46.3} \%&
{\scriptsize .} ($\pm$ 0.36) & {\scriptsize $~$ 56.2} \%&
{\scriptsize .} ($\pm$ 0.13) & {\scriptsize $~$ 39.9} \%\\
CST (Ours, SGD) $c=0.3$ & $\bsy\times$ &
{\scriptsize .} ($\pm$ 0.07) & {\scriptsize $~$ 68.3} \%& \textbf{{\scriptsize .} ($\pm$ 0.40)} & {\scriptsize $~$ .} \%& \textbf{{\scriptsize .} ($\pm$ 0.23)} & {\scriptsize $~$ 72.9} \%\\
CST (Ours, SGD) $c=0.5$ & $\bsy\times$ &
\textbf{{\scriptsize .} ($\pm$ 0.02)} & {\scriptsize $~$ 88.9} \%& {\scriptsize . ($\pm$ 0.92)} & {\scriptsize 111.0} \%& {\scriptsize .} ($\pm$ 0.13) & {\scriptsize $~$ 95.8} \%\\

\cmidrule{1-8}
CST (Ours, Adam) $c=0.03$ & $\bsy\times$ &
{\scriptsize 92.7} ($\pm$ 0.06) & \textbf{{\scriptsize $~$ 37.4}} \%&
{\scriptsize 65.6} ($\pm$ 0.63) & \textbf{{\scriptsize $~$ 39.4}} \%&
{\scriptsize 90.1} ($\pm$ 0.10) & \textbf{{\scriptsize $~$ 24.2}} \%\\
CST (Ours, Adam) $c=0.1$ & $\bsy\times$ &
{\scriptsize 93.9} ($\pm$ 0.09) & {\scriptsize $~$ 46.3} \%&
{\scriptsize 72.2} ($\pm$ 0.36) & {\scriptsize $~$ 56.2} \%&
{\scriptsize 91.3} ($\pm$ 0.13) & {\scriptsize $~$ 39.9} \%\\
CST (Ours, Adam) $c=0.3$ & $\bsy\times$ &
{\scriptsize 94.7} ($\pm$ 0.07) & {\scriptsize $~$ 68.3} \%& \textbf{{\scriptsize 73.5} ($\pm$ 0.40)} & {\scriptsize $~$ 97.4} \%& \textbf{{\scriptsize 91.7} ($\pm$ 0.23)} & {\scriptsize $~$ 72.9} \%\\
CST (Ours, Adam) $c=0.5$ & $\bsy\times$ &
\textbf{{\scriptsize 94.8} ($\pm$ 0.02)} & {\scriptsize $~$ 88.9} \%& {\scriptsize 72.5 ($\pm$ 0.92)} & {\scriptsize 111.0} \%& {\scriptsize 91.5} ($\pm$ 0.13) & {\scriptsize $~$ 95.8} \%\\
\cmidrule{1-8}
MTL &$\bsy\times$& {\scriptsize 96.7 $\dagger$} & {\scriptsize 100.0} \%& {\scriptsize 79.6 $\dagger$} & {\scriptsize 100.0} \%& {\scriptsize 91.5 $\dagger$} & {\scriptsize 100.0} \%\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main_opt_table}
\end{center}
\end{table*}




==> materials/9_backup/6_app_main_table_epoch.tex <==
\begin{table*}[t]
\tiny
\begin{center}
\caption{\small Performance comparison of the proposed method and other baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (Accuracy) and average forgetting (Forgetting) across $5$ independent runs. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Values with $\dagger$ $~$ denote reported performances from \cite{Saha2021}. PackNet~\cite{mallya2018packnet} is baseline.}

\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Method}}&\multicolumn{2}{c}{\textbf{Permuted MNIST}} & \multicolumn{2}{c}{\textbf{Split CIFAR-100}} & \multicolumn{2}{c}{\textbf{5 Datasets}} \\


\midrule
& CF & Accuracy & Capacity Used & Accuracy & Capacity Used & Accuracy & Capacity Used\\
\midrule
CST (Ours, epoch=10) $c=0.03$ & $\bsy\times$ &
{\scriptsize .} ($\pm$ 0.06) & \textbf{{\scriptsize $~$ 37.4}} \%&
{\scriptsize .} ($\pm$ 0.63) & \textbf{{\scriptsize $~$ 39.4}} \%&
{\scriptsize .} ($\pm$ 0.10) & \textbf{{\scriptsize $~$ 24.2}} \%\\
CST (Ours, Adam, epoch=10) $c=0.1$ & $\bsy\times$ &
{\scriptsize .} ($\pm$ 0.09) & {\scriptsize $~$ 46.3} \%&
{\scriptsize .} ($\pm$ 0.36) & {\scriptsize $~$ 56.2} \%&
{\scriptsize .} ($\pm$ 0.13) & {\scriptsize $~$ 39.9} \%\\
CST (Ours, Adam, epoch=10) $c=0.3$ & $\bsy\times$ &
{\scriptsize .} ($\pm$ 0.07) & {\scriptsize $~$ 68.3} \%& \textbf{{\scriptsize .} ($\pm$ 0.40)} & {\scriptsize $~$ .} \%& \textbf{{\scriptsize .} ($\pm$ 0.23)} & {\scriptsize $~$ 72.9} \%\\
CST (Ours, Adam, epoch=10) $c=0.5$ & $\bsy\times$ &
\textbf{{\scriptsize .} ($\pm$ 0.02)} & {\scriptsize $~$ 88.9} \%& {\scriptsize . ($\pm$ 0.92)} & {\scriptsize 111.0} \%& {\scriptsize .} ($\pm$ 0.13) & {\scriptsize $~$ 95.8} \%\\

\cmidrule{1-8}
CST (Ours, Adam, epoch=50) $c=0.03$ & $\bsy\times$ &
{\scriptsize 92.7} ($\pm$ 0.06) & \textbf{{\scriptsize $~$ 37.4}} \%&
{\scriptsize 65.6} ($\pm$ 0.63) & \textbf{{\scriptsize $~$ 39.4}} \%&
{\scriptsize 90.1} ($\pm$ 0.10) & \textbf{{\scriptsize $~$ 24.2}} \%\\
CST (Ours, Adam, epoch=50) $c=0.1$ & $\bsy\times$ &
{\scriptsize 93.9} ($\pm$ 0.09) & {\scriptsize $~$ 46.3} \%&
{\scriptsize 72.2} ($\pm$ 0.36) & {\scriptsize $~$ 56.2} \%&
{\scriptsize 91.3} ($\pm$ 0.13) & {\scriptsize $~$ 39.9} \%\\
CST (Ours, Adam, epoch=50) $c=0.3$ & $\bsy\times$ &
{\scriptsize 94.7} ($\pm$ 0.07) & {\scriptsize $~$ 68.3} \%& \textbf{{\scriptsize 73.5} ($\pm$ 0.40)} & {\scriptsize $~$ 97.4} \%& \textbf{{\scriptsize 91.7} ($\pm$ 0.23)} & {\scriptsize $~$ 72.9} \%\\
CST (Ours, Adam, epoch=50) $c=0.5$ & $\bsy\times$ &
\textbf{{\scriptsize 94.8} ($\pm$ 0.02)} & {\scriptsize $~$ 88.9} \%& {\scriptsize 72.5 ($\pm$ 0.92)} & {\scriptsize 111.0} \%& {\scriptsize 91.5} ($\pm$ 0.13) & {\scriptsize $~$ 95.8} \%\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main_epoch_table}
\end{center}
\end{table*}




==> materials/9_backup/6_app_main_table_new.tex <==
\begin{table*}[t]
\tiny
\begin{center}
\caption{\small (PMNIST, 5-Datasets, Omniglot Rotation) Performance comparison of the proposed method and other baselines on various benchmark datasets. We report the mean and standard-deviation of the average accuracy (Accuracy) and average forgetting (Forgetting) across $5$ independent runs. CF indicates that the method suffers from the catastrophic forgetting. The best results are highlighted in bold. Values with $\dagger$ $~$ denote reported performances from \cite{Saha2021}. PackNet~\cite{mallya2018packnet} is baseline.}

\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular}{lccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Method}}&
% \multicolumn{3}{c}{\textbf{Permuted MNIST}} & 
\multicolumn{3}{c}{\textbf{Split CIFAR-100}} & 
\multicolumn{3}{c}{\textbf{Split CIFAR-100 Superclass}} \\ 
% \multicolumn{3}{c}{\textbf{5 Datasets}} & 
% \multicolumn{3}{c}{\textbf{Omniglot Rotation}} \\


\midrule
& CF & 
% ACC (\%) & CAP (\%) & BWT (\%) & 
ACC (\%) & CAP (\%) & BWT & 
% ACC (\%) & CAP (\%) & BWT (\%) & 
% ACC (\%) & CAP (\%) & BWT (\%) & 
ACC (\%) & CAP (\%) & BWT \\
\midrule
STL & $\bsy\times$ &
% {\scriptsize 97.6} ($\pm$ 0.10) & {\scriptsize 1000.0} \%& & 
% {\scriptsize 70.9} ($\pm$ 0.38) & {\scriptsize 1000.0} \%& & 
% {\scriptsize 90.7} ($\pm$ 0.53) & {\scriptsize 500.0} \% & &
% & & & 
% & & \\
% {\scriptsize 97.2} ($\pm$ 0.11) & {\scriptsize $~$ 1000} ($\pm$ 0.0) & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 73.9} ($\pm$ 0.44) & {\scriptsize $~$ 1000} ($\pm$ 0.0) & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 62.0} ($\pm$ 0.44) & {\scriptsize $~$ 2000} ($\pm$ 0.0) & {\scriptsize 0.0} ($\pm$ 0.0) \\
% {\scriptsize 93.4} ($\pm$ 0.12) & {\scriptsize $~$ 500} ($\pm$ 0.0) & {\scriptsize 0.0} ($\pm$ 0.0) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
 \midrule
FINETUNE&  \checkmark &
% {\scriptsize 62.5} ($\pm$ 2.96) & {\scriptsize 100.0} \%& &
% {\scriptsize 13.2} ($\pm$ 0.54) & {\scriptsize 100.0} \%& &
% {\scriptsize 36.8} ($\pm$ 2.25) & {\scriptsize 100.0} \%& & 
% & & & 
% & & \\
% {\scriptsize 30.4} ($\pm$ 2.82) & {\scriptsize $~$ 100} ($\pm$ 0.0) & {\scriptsize -73.5} ($\pm$ 3.14) &
{\scriptsize 57.1} ($\pm$ 1.1) & {\scriptsize $~$ 100.0} ($\pm$ 0.0) & {\scriptsize -0.22} ($\pm$ 0.01) &
{\scriptsize 37.3} ($\pm$ 1.6) & {\scriptsize $~$ 100.0} ($\pm$ 0.0) & {\scriptsize -0.28} ($\pm$ 0.02) \\
% {\scriptsize 56.9} ($\pm$ 0.91) & {\scriptsize $~$ 100} ($\pm$ 0.0) & {\scriptsize -45.4} ($\pm$ 1.16) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
HAT~\cite{Serra2018} &  \checkmark &
% {\scriptsize -}  & {\scriptsize -} & &
% {\scriptsize 72.0} $\dagger$ & {\scriptsize 100.0} \%& &
% {\scriptsize 88.6} $\dagger$ & {\scriptsize 100.0} \%& &
% & & &
% & & \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize 72.1} ($\pm$ 0.50) $\dagger$ & {\scriptsize $~$ 100.0} ($\pm$ 0.0) & {\scriptsize -0.00} ($\pm$ 0.00) $\dagger$ &
{\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
APD~\cite{Yoon2020}  & \checkmark &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize 56.8} ($\pm$ 0.33) $\dagger$ & {\scriptsize x.xx} \%& {\scriptsize -} ($\pm$ -) \\
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} \%& {\scriptsize -} ($\pm$ -) \\

AGS-CL~\cite{Jung2020} & \checkmark &
% {\scriptsize 91.1} ($\pm$ 0.71) & {\scriptsize 100.0} \%& &
% {\scriptsize 49.6} ($\pm$ 1.89) & {\scriptsize 100.0} \%& &
% {\scriptsize -}  & - & &
% & & & 
% & & \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
GPM~\cite{Saha2021} & \checkmark &
% {\scriptsize 92.9} ($\pm$ 0.20) & {\scriptsize x.xx} \%&
% {\scriptsize 93.9} $\dagger$ & {\scriptsize 100.0} \%& &
% {\scriptsize 72.5} $\dagger$ & {\scriptsize 100.0} \%& &
% {\scriptsize 91.3} $\dagger$ & {\scriptsize 100.0} \%& &
% & & & 
% & & \\
% {\scriptsize 93.9} ($\pm$ 0.16) $\dagger$ & \textbf{{\scriptsize $~$ 100} ($\pm$ 0.00)} & {\scriptsize -0.03} ($\pm$ 0.00) &
{\scriptsize 72.5} ($\pm$ 0.40) $\dagger$ & {\scriptsize $~$ 100.0} ($\pm$ 0.00) & {\scriptsize -0.00} ($\pm$ 0.00) &
{\scriptsize 57.7} ($\pm$ 0.37) $\dagger$ & {\scriptsize $~$ 100.0} ($\pm$ 0.00) & {\scriptsize -0.01} ($\pm$ 0.00) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
\midrule
PackNet~\cite{mallya2018packnet}  & $\bsy\times$ &
%\textbf{{\scriptsize 95.9} ($\pm$ 0.05)} & {\scriptsize $~$ 96.8} \%& % 0.655 + 10*1/32
% {\scriptsize 94.5} ($\pm$ 0.05) & {\scriptsize $~$ 72.1} \%& & % 0.408 + 10*1/32
% {\scriptsize 58.3} ($\pm$ 0.46) & {\scriptsize 131.2} \%& & % 0.999 + 10*1/32
% {\scriptsize 89.0} ($\pm$ 0.21) & {\scriptsize 115.4} \%& & % 0.998 + 5 * 1/32 
% & & & 
% & & \\ 
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize 72.5} ($\pm$ 0.21) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
{\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\
% LL-Ticket~\cite{longliveticket}  & $\bsy\times$ &
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%&
% {\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize $~$ x.xx} \%\\
\midrule
CST (Ours) $c=0.03$ & $\bsy\times$ & % need to add per-task sparsity
% {\scriptsize 95.0} ($\pm$ 0.11) & \textbf{{\scriptsize $~$ 13.1} ($\pm$ 0.06)} & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 71.0} ($\pm$ 0.56) & \textbf{{\scriptsize $~$ 11.7} ($\pm$ 0.25)} & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 62.5} ($\pm$ 0.40) & \textbf{{\scriptsize $~$ 10.4} ($\pm$ 0.24)} & {\scriptsize 0.0} ($\pm$ 0.0) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\

CST (Ours) $c=0.05$ & $\bsy\times$ & % need to add per-task sparsity
% {\scriptsize 95.6} ($\pm$ 0.15) & {\scriptsize $~$ 19.5} ($\pm$ 0.33) & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 72.4} ($\pm$ 0.44) & {\scriptsize $~$ 18.3} ($\pm$ 0.54) & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 63.1} ($\pm$ 0.16) & {\scriptsize $~$ 14.9} ($\pm$ 0.63) & {\scriptsize 0.0} ($\pm$ 0.0) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\

CST (Ours) $c=0.1$ & $\bsy\times$ & % need to add per-task sparsity
% {\scriptsize 96.2} ($\pm$ 0.10) & {\scriptsize $~$ 33.8} ($\pm$ 0.44) & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 74.7} ($\pm$ 0.33) & {\scriptsize $~$ 32.7} ($\pm$ 0.75) & {\scriptsize 0.0} ($\pm$ 0.0) &
\textbf{{\scriptsize 63.7} ($\pm$ 0.39)} & {\scriptsize $~$ 22.9} ($\pm$ 1.56) & \textbf{{\scriptsize 0.0} ($\pm$ 0.0)} \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\

CST (Ours) $c=0.3$ & $\bsy\times$ & % need to add per-task sparsity
% \textbf{{\scriptsize 96.5} ($\pm$ 0.06)} & {\scriptsize $~$ 70.2} ($\pm$ 0.50) & \textbf{{\scriptsize 0.0} ($\pm$ 0.0)} &
{\scriptsize 76.4} ($\pm$ 0.38) & {\scriptsize $~$ 73.1} ($\pm$ 0.81) & {\scriptsize 0.0} ($\pm$ 0.0) &
{\scriptsize 63.4} ($\pm$ 0.26) & {\scriptsize $~$ 38.2} ($\pm$ 0.74) & {\scriptsize 0.0} ($\pm$ 0.0) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\

CST (Ours) $c=0.5$ & $\bsy\times$ & % need to add per-task sparsity
% {\scriptsize 96.3} ($\pm$ 0.08) & {\scriptsize $~$ 90.9} ($\pm$ 0.31) & {\scriptsize 0.0} ($\pm$ 0.0) &
\textbf{{\scriptsize 76.5} ($\pm$ 0.39)} & {\scriptsize $~$ 92.2} ($\pm$ 0.75) & \textbf{{\scriptsize 0.0} ($\pm$ 0.0)} &
{\scriptsize 63.4} ($\pm$ 0.17) & {\scriptsize $~$ 57.0} ($\pm$ 0.63) & {\scriptsize 0.0} ($\pm$ 0.0) \\
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) &
% {\scriptsize -} ($\pm$ -) & \textbf{{\scriptsize $~$ -}} \%& {\scriptsize -} ($\pm$ -) \\

\midrule
MTL &$\bsy\times$& 
% {\scriptsize 96.7 $\dagger$} & {\scriptsize 100.0} \% & {\scriptsize -} & 
{\scriptsize 79.6 $\dagger$} & {\scriptsize 100} & {\scriptsize -} & 
% {\scriptsize 91.5 $\dagger$} & {\scriptsize 100.0} \% & {\scriptsize -} \\
{\scriptsize 61.0 $\dagger$} & {\scriptsize 100} & {\scriptsize -} \\ 
% {\scriptsize -} & {\scriptsize -} \% & {\scriptsize -} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main_table}
\end{center}
\end{table*}




==> materials/9_backup/6_app_plots_acc_vs_cap.tex <==
\begin{figure}[ht]
    \centering
    \vspace{-0.1in}
    \renewcommand{\arraystretch}{1}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    \includegraphics[width=.5\columnwidth]{images/5_acc_vs_cap_pmnist_new_w_dots_no_title.pdf} &
    \includegraphics[width=.5\columnwidth]{images/5_acc_vs_cap_omniglot_rotation_new_wo_packnet_w_dots_no_title.pdf} \\
    % \vspace{-0.06in}
    \small (a) PMNIST - MLP & \small (b) Omniglot Rotation - LeNet \\
    % \vspace{-0.06in}
    \end{tabular}}
    % \vspace{-0.15in}
    \caption{\footnotesize \textbf{Accuracy over Total Capacity Usage}: WSN achieves best performance under Accuracy-Capacity trade-off in PMNIST and Omniglot Rotation datasets - It can be seen that WSN's accuracy is higher than other competing baselines, especially PackNet, while utilizing less total capacity.}
    \label{fig:acc_vs_cap_appendix}
    % \vspace{-0.1in}
\end{figure}

==> materials/9_backup/7_main_confusion_5data.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    \setlength{\tabcolsep}{-10pt}{%
    \begin{tabular}{cccc}
    
    \includegraphics[height=3.6cm]{images/corr_binary_5-Dataset_seed_5_capacity_5.pdf} &~
    \includegraphics[height=3.6cm]{images/corr_binary_5-Dataset_seed_1_capacity_10.pdf} &~ 
    \includegraphics[height=3.6cm]{images/corr_binary_5-Dataset_seed_3_capacity_30.pdf} &~
    \includegraphics[height=3.6cm]{images/corr_binary_5-Dataset_seed_3_capacity_50.pdf} \\ 
    
    % plot captions
    \small (a) $c=0.05$ & \small (b) $c=0.1$ & 
    \small (c) $c=0.3$ & \small (d) $c=0.5$ \\
    \end{tabular}
    %\end{adjustbox}
    }
    \caption{\footnotesize \textbf{Average Binary Map Correlation} on Sequence of 5-Dataset Experiments: the binary maps get overlapped with prior ones as the number of tasks increases..}
    \label{fig:main_5_data_conf}
\end{figure*}

==> materials/9_backup/7_main_confusion_omniglot.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    \setlength{\tabcolsep}{-9pt}{%
    \begin{tabular}{cccc}
    
    \includegraphics[height=3.45cm]{images/corr_binary_Omniglot Rotation_seed_5_capacity_5.pdf} &~\;\;
    \includegraphics[height=3.45cm]{images/corr_binary_Omniglot Rotation_seed_1_capacity_10.pdf} &~\;\; 
    \includegraphics[height=3.45cm]{images/corr_binary_Omniglot Rotation_seed_3_capacity_30.pdf} &~\;\;
    \includegraphics[height=3.45cm]{images/corr_binary_Omniglot Rotation_seed_9_capacity_50.pdf} \\ 
    
    % plot captions
    \small (a) $c=0.05$ & \small (b) $c=0.1$ & 
    \small (c) $c=0.3$ & \small (d) $c=0.5$ \\
    \end{tabular}
    %\end{adjustbox}
    }
    \caption{\footnotesize \textbf{Average Binary Map Correlation} on Sequence of Omniglot Rotation Experiments: the binary maps get overlapped with prior ones as the number of tasks increases..}
    \label{fig:main_omniglot_conf}
\end{figure*}

==> materials/9_backup/7_main_confusion_pmnist.tex <==
\begin{figure*}[ht]
    \centering
    %\begin{adjustbox}{width=0.5\textwidth}
    \setlength{\tabcolsep}{-10pt}{%
    \begin{tabular}{cccc}
    
    \includegraphics[height=3.6cm]{images/corr_binary_PMNIST_seed_2_capacity_5.pdf} &~
    \includegraphics[height=3.6cm]{images/corr_binary_PMNIST_seed_4_capacity_10.pdf} &~ 
    \includegraphics[height=3.6cm]{images/corr_binary_PMNIST_seed_3_capacity_30.pdf} &~
    \includegraphics[height=3.6cm]{images/corr_binary_PMNIST_seed_4_capacity_50.pdf} \\ 
    
    % plot captions
    \small (a) $c=0.05$ & \small (b) $c=0.1$ & 
    \small (c) $c=0.3$ & \small (d) $c=0.5$ \\
    \end{tabular}
    %\end{adjustbox}
    }
    \caption{\footnotesize \textbf{Average Binary Map Correlation} on Sequence of PMNIST Experiments: the binary maps get overlapped with prior ones as the number of tasks increases..}
    \label{fig:main_pmnist_conf}
\end{figure*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak
